A Uniformly Selected Sample of Low-mass Black Holes in Seyfert 1 Galaxies

We have conducted a systematic search of low-mass black holes (BHs) in active galactic nuclei (AGNs) with broad Halpha emission lines, aiming at building a homogeneous sample that is more complete than previous ones for fainter, less highly accreting sources. For this purpose, we developed a set of elaborate, automated selection procedures and applied it uniformly to the Fourth Data Release of the Sloan Digital Sky Survey. Special attention is given to AGN--galaxy spectral decomposition and emission-line deblending. We define a sample of 309 type 1 AGNs with BH masses in the range $8 \times 10^4$--$2 \times 10^6$ \msun (with a median of $1.2 \times 10^6$ solar mass), using the virial mass estimator based on the broad Halpha line. About half of our sample of low-mass BHs differs from that of Greene & Ho, with 61 of them discovered here for the first time. Our new sample picks up more AGNs with low accretion rates: the Eddington ratios of the present sample range from $<~0.01$ to ~1, with 30% below 0.1. This suggests that a significant fraction of low-mass BHs in the local Universe are accreting at low rates. The host galaxies of the low-mass BHs have luminosities similar to those of $L^*$ field galaxies, optical colors of Sbc spirals, and stellar spectral features consistent with a continuous star formation history with a mean stellar age of less than 1 Gyr.

==> full_table1.tex <==
%ID & NAME                  & z      & PTROg & G_R  & A_g        % SPEC
1   & J000111.15$-$100155.7 & 0.0489 & 18.65 & 0.78 & 0.15   \\  % 52143-0650-174
2   & J000308.48$+$154842.2 & 0.1175 & 18.31 & 0.55 & 0.14   \\  % 52235-0750-609
3   & J001728.84$-$001826.8 & 0.1118 & 17.85 & 0.74 & 0.10   \\  % 51795-0389-120
4   & J002629.13$+$000509.6 & 0.2133 & 19.64 & 0.80 & 0.09   \\  % 51900-0390-624
5   & J003108.82$+$144543.4 & 0.1188 & 18.63 & 0.95 & 0.24   \\  % 51821-0417-182
6   & J004042.10$-$110957.7 & 0.0273 & 17.62 & 0.71 & 0.10   \\  % 52162-0655-089
7   & J005633.36$+$000510.2 & 0.0792 & 19.50 & 0.52 & 0.10   \\  % 51913-0394-624
8   & J005842.93$-$094102.4 & 0.1887 & 20.11 & 0.66 & 0.15   \\  % 52146-0658-488
9   & J010600.57$+$152441.9 & 0.2043 & 19.63 & 0.39 & 0.26   \\  % 51811-0422-321
10  & J010712.04$+$140845.0 & 0.0768 & 18.49 & 0.62 & 0.26   \\  % 51811-0422-224
11  & J011749.81$-$100114.7 & 0.1410 & 19.37 & 0.58 & 0.15   \\  % 52177-0660-142
12  & J012058.24$-$000709.1 & 0.1659 & 19.77 & 0.67 & 0.13   \\  % 51817-0399-317
13  & J012150.64$-$100510.0 & 0.1033 & 18.18 & 0.73 & 0.13   \\  % 52163-0661-229
14  & J012423.99$+$134325.4 & 0.2551 & 19.18 & 0.48 & 0.16   \\  % 51893-0424-097
15  & J014816.21$+$125018.0 & 0.1570 & 20.14 & 0.92 & 0.23   \\  % 51820-0429-084
16  & J020307.71$+$140816.9 & 0.0594 & 17.45 & 0.67 & 0.34   \\  % 51900-0427-492
17  & J022756.28$+$005733.2 & 0.1282 & 18.88 & 0.61 & 0.11   \\  % 51820-0407-329
18  & J022849.52$-$090153.9 & 0.0720 & 18.25 & 0.55 & 0.10   \\  % 51908-0454-109
19  & J024402.24$-$091540.9 & 0.1216 & 18.41 & 0.66 & 0.10   \\  % 51910-0456-257
20  & J024912.87$-$081525.7 & 0.0294 & 16.54 & 0.67 & 0.11   \\  % 51910-0456-077
21  & J030417.78$+$002827.4 & 0.0445 & 15.88 & 0.53 & 0.30   \\  % 51817-0411-513
22  & J031743.12$+$001936.9 & 0.0687 & 17.44 & 0.42 & 0.34   \\  % 51929-0413-470
23  & J032515.59$+$003408.4 & 0.1020 & 19.51 & 0.71 & 0.50   \\  % 51901-0414-405
24  & J032606.77$+$011429.7 & 0.1274 & 17.89 & 0.73 & 0.42   \\  % 51901-0414-426
25  & J032707.33$-$075639.4 & 0.1538 & 19.42 & 0.54 & 0.18   \\  % 51924-0460-014
26  & J034141.07$-$055315.4 & 0.1773 & 18.70 & 0.53 & 0.20   \\  % 51909-0462-504
27  & J073106.87$+$392644.7 & 0.0485 & 16.23 & 0.63 & 0.22   \\  % 53034-1734-137
28  & J073631.82$+$383058.3 & 0.0733 & 17.66 & 0.67 & 0.23   \\  % 51877-0431-533
29  & J073956.03$+$402816.3 & 0.0611 & 17.75 & 0.69 & 0.17   \\  % 51884-0432-384
30  & J074251.09$+$333403.9 & 0.1255 & 19.07 & 0.88 & 0.19   \\  % 51959-0541-617
31  & J074423.45$+$243046.3 & 0.1167 & 17.86 & 0.73 & 0.21   \\  % 52314-0857-039
32  & J074424.48$+$332034.8 & 0.0633 & 17.28 & 0.71 & 0.17   \\  % 51959-0541-602
33  & J074659.82$+$440728.8 & 0.0758 & 16.72 & 0.63 & 0.15   \\  % 53052-1736-062
34  & J074810.37$+$454003.1 & 0.1428 & 17.94 & 0.73 & 0.23   \\  % 53055-1737-220
35  & J074831.91$+$464455.5 & 0.0887 & 19.68 & 0.53 & 0.30   \\  % 53055-1737-468
36  & J074948.33$+$264734.2 & 0.1316 & 18.61 & 0.97 & 0.13   \\  % 52316-0858-438
37  & J075038.12$+$315737.1 & 0.0548 & 16.70 & 0.69 & 0.23   \\  % 52583-0890-400
38  & J075709.34$+$423616.4 & 0.0740 & 17.32 & 0.67 & 0.17   \\  % 51869-0437-274
39  & J080303.63$+$515729.1 & 0.0701 & 17.77 & 0.38 & 0.19   \\  % 53090-1780-369
40  & J080352.99$+$263123.4 & 0.0463 & 16.23 & 0.49 & 0.16   \\  % 52670-1205-330
41  & J080511.91$+$064119.5 & 0.0996 & 18.65 & 0.58 & 0.11   \\  % 53080-1756-305
42  & J080537.37$+$362522.1 & 0.0885 & 17.46 & 0.71 & 0.19   \\  % 52253-0758-109
43  & J080629.81$+$241955.7 & 0.0414 & 16.42 & 0.52 & 0.17   \\  % 52705-1265-139
44  & J080743.73$+$345454.4 & 0.1077 & 18.31 & 0.72 & 0.17   \\  % 52378-0892-244
45  & J080907.57$+$441641.5 & 0.0539 & 17.73 & 0.54 & 0.15   \\  % 51877-0439-216
46  & J081207.99$+$320453.1 & 0.0616 & 18.08 & 0.71 & 0.16   \\  % 52318-0861-430
47  & J081547.55$+$324213.7 & 0.1100 & 18.77 & 0.67 & 0.16   \\  % 52325-0862-287
48  & J081550.24$+$250641.0 & 0.0727 & 17.93 & 0.52 & 0.15   \\  % 52709-1266-109
49  & J081825.15$+$472950.3 & 0.0538 & 18.29 & 0.73 & 0.19   \\  % 51868-0441-438
50  & J081856.38$+$454908.2 & 0.2277 & 19.56 & 0.78 & 0.16   \\  % 51868-0441-106
51  & J082050.03$+$243909.1 & 0.1300 & 19.20 & 0.50 & 0.12   \\  % 52962-1585-549
52  & J082325.92$+$065106.5 & 0.0725 & 16.97 & 0.50 & 0.09   \\  % 52962-1296-371
53  & J082326.68$+$513605.2 & 0.1363 & 17.86 & 0.66 & 0.17   \\  % 51882-0442-420
54  & J082433.33$+$380013.1 & 0.1031 & 16.93 & 0.50 & 0.16   \\  % 52589-0893-636
55  & J082502.16$+$082614.9 & 0.0824 & 18.54 & 0.81 & 0.15   \\  % 53084-1758-332
56  & J082737.40$+$272917.3 & 0.1542 & 18.53 & 0.51 & 0.12   \\  % 52932-1267-107
57  & J082912.68$+$500652.3 & 0.0434 & 17.69 & 0.42 & 0.16   \\  % 51873-0443-514
58  & J083019.66$+$084725.1 & 0.0771 & 17.35 & 0.65 & 0.12   \\  % 53084-1758-524
59  & J083211.58$+$502408.6 & 0.1719 & 19.93 & 0.59 & 0.15   \\  % 51873-0445-301
60  & J083346.04$+$062026.6 & 0.1095 & 18.13 & 0.43 & 0.14   \\  % 52963-1297-154
61  & J083803.68$+$540642.1 & 0.0295 & 18.03 & 0.79 & 0.13   \\  % 51899-0446-271
62  & J083928.45$+$082102.4 & 0.1305 & 18.42 & 0.53 & 0.24   \\  % 53081-1759-148
63  & J084011.28$+$075915.8 & 0.1321 & 18.54 & 0.79 & 0.25   \\  % 52964-1298-335
64  & J084303.60$+$361011.2 & 0.0871 & 17.22 & 0.56 & 0.14   \\  % 52320-0864-067
65  & J084719.80$+$380043.7 & 0.1363 & 18.18 & 0.49 & 0.12   \\  % 52323-0865-191
66  & J084739.61$+$360444.4 & 0.0866 & 17.88 & 0.63 & 0.11   \\  % 52672-0934-517
67  & J085152.63$+$522833.0 & 0.0645 & 16.36 & 0.43 & 0.10   \\  % 51877-0447-554
68  & J085259.11$+$412203.0 & 0.1348 & 18.21 & 0.69 & 0.11   \\  % 52293-0830-239
69  & J085655.29$+$442653.4 & 0.1791 & 18.88 & 0.72 & 0.10   \\  % 52605-0897-178
70  & J085836.04$+$353634.3 & 0.1258 & 17.96 & 0.55 & 0.11   \\  % 52964-1211-420
71  & J085906.36$+$542150.2 & 0.1819 & 19.63 & 0.82 & 0.06   \\  % 51900-0449-571
72  & J090031.76$+$432709.0 & 0.0609 & 17.69 & 0.70 & 0.07   \\  % 52294-0831-464
73  & J090320.97$+$045738.1 & 0.0570 & 17.83 & 0.54 & 0.13   \\  % 52649-1192-183
74  & J090431.22$+$075330.9 & 0.0838 & 18.22 & 0.48 & 0.20   \\  % 52973-1300-127
75  & J090731.06$+$445428.5 & 0.1160 & 19.68 & 0.70 & 0.07   \\  % 52312-0832-397
76  & J091045.91$+$480339.4 & 0.1057 & 18.92 & 0.45 & 0.07   \\  % 52620-0899-367
77  & J091102.33$+$550023.1 & 0.0443 & 17.57 & 0.75 & 0.07   \\  % 51908-0450-108
78  & J091449.06$+$085321.1 & 0.1402 & 18.65 & 0.55 & 0.16   \\  % 52976-1301-471
79  & J091536.77$+$062540.6 & 0.3419 & 19.59 & 0.32 & 0.14   \\  % 52652-1193-563
80  & J091624.82$+$383433.5 & 0.2117 & 19.75 & 0.63 & 0.08   \\  % 52707-0937-066
81  & J091858.97$+$053844.3 & 0.1906 & 18.81 & 0.54 & 0.16   \\  % 52707-0991-391
82  & J091917.89$+$050953.0 & 0.0749 & 16.41 & 0.56 & 0.21   \\  % 52707-0991-268
83  & J092209.74$-$003222.4 & 0.0561 & 16.46 & 0.72 & 0.12   \\  % 52000-0474-225
84  & J092411.46$+$022321.8 & 0.0894 & 17.63 & 0.81 & 0.21   \\  % 51929-0473-619
85  & J092547.32$+$050231.7 & 0.1267 & 19.42 & 0.43 & 0.19   \\  % 52707-0991-061
86  & J092700.53$+$084329.5 & 0.1124 & 18.67 & 0.91 & 0.20   \\  % 53050-1303-300
87  & J093308.89$+$534749.0 & 0.0573 & 17.06 & 0.58 & 0.05   \\  % 52266-0555-049
88  & J093749.85$+$585522.7 & 0.1323 & 19.00 & 0.69 & 0.07   \\  % 51915-0453-310
89  & J093829.39$+$034826.7 & 0.1192 & 18.84 & 0.59 & 0.14   \\  % 52264-0569-634
90  & J093836.00$+$383613.4 & 0.1511 & 19.69 & 0.59 & 0.06   \\  % 52725-1215-114
91  & J094258.55$+$083810.1 & 0.1341 & 18.07 & 0.50 & 0.13   \\  % 52724-1234-390
92  & J094310.12$+$604559.2 & 0.0743 & 18.32 & 0.58 & 0.09   \\  % 51910-0486-059
93  & J094529.37$+$093610.4 & 0.0133 & 15.30 & 0.70 & 0.09   \\  % 52757-1305-179
94  & J095053.97$+$632145.7 & 0.0873 & 18.35 & 0.93 & 0.14   \\  % 51943-0487-424
95  & J095151.82$+$060143.7 & 0.0933 & 18.38 & 0.79 & 0.13   \\  % 52725-0994-490
96  & J095306.81$+$365028.1 & 0.0491 & 16.53 & 0.32 & 0.05   \\  % 52998-1596-344
97  & J095330.54$+$562653.5 & 0.0660 & 17.91 & 0.70 & 0.04   \\  % 52317-0558-282
98  & J095438.79$+$403204.3 & 0.0676 & 18.57 & 0.34 & 0.05   \\  % 52709-1216-120
99  & J095553.98$+$534846.1 & 0.3037 & 20.30 & 0.48 & 0.04   \\  % 52282-0769-062
100 & J095835.99$-$005942.6 & 0.1669 & 19.21 & 0.70 & 0.15   \\  % 51633-0268-085
101 & J100510.52$+$543255.5 & 0.0499 & 17.59 & 0.79 & 0.03   \\  % 52652-0945-172
102 & J100617.52$+$365703.1 & 0.1090 & 18.89 & 0.51 & 0.05   \\  % 52993-1426-132
103 & J100711.44$+$581714.3 & 0.2020 & 19.71 & 0.81 & 0.03   \\  % 52317-0558-611
104 & J101108.40$+$002908.7 & 0.1000 & 19.33 & 0.59 & 0.14   \\  % 51909-0270-490
105 & J101627.34$-$000714.6 & 0.0944 & 19.32 & 0.66 & 0.13   \\  % 51883-0271-277
106 & J101748.42$+$405116.4 & 0.0939 & 18.35 & 0.80 & 0.06   \\  % 53034-1357-543
107 & J102124.88$+$012720.3 & 0.0669 & 17.23 & 0.74 & 0.22   \\  % 51999-0503-098
108 & J102212.61$+$383742.8 & 0.0559 & 18.38 & 0.68 & 0.07   \\  % 52998-1428-232
109 & J102235.15$+$022930.5 & 0.0698 & 18.03 & 0.56 & 0.16   \\  % 51999-0503-585
110 & J102348.44$+$040553.7 & 0.0989 & 17.35 & 0.62 & 0.12   \\  % 52319-0575-199
111 & J102703.91$+$485023.9 & 0.1474 & 18.23 & 0.82 & 0.03   \\  % 52338-0874-499
112 & J103234.85$+$650227.9 & 0.0057 & 13.42 & 0.55 & 0.06   \\  % 51930-0489-193
113 & J103247.19$+$114521.2 & 0.1130 & 19.15 & 0.75 & 0.16   \\  % 53089-1599-555
114 & J103618.78$+$051958.1 & 0.1845 & 19.67 & 0.55 & 0.10   \\  % 52367-0577-414
115 & J103759.26$+$615310.8 & 0.0697 & 16.13 & 0.51 & 0.03   \\  % 52376-0773-258
116 & J103928.73$+$562058.2 & 0.0746 & 18.82 & 0.46 & 0.02   \\  % 52428-0948-259
117 & J104210.03$-$001814.8 & 0.1147 & 18.84 & 0.50 & 0.19   \\  % 51910-0275-312
118 & J104504.24$+$114508.8 & 0.0548 & 16.87 & 0.62 & 0.09   \\  % 53115-1601-427
119 & J104842.45$+$413302.3 & 0.0629 & 16.97 & 0.62 & 0.05   \\  % 53047-1361-020
120 & J105131.91$+$504223.2 & 0.1321 & 18.98 & 0.66 & 0.05   \\  % 52669-0876-497
121 & J105424.29$+$454130.5 & 0.0637 & 17.32 & 0.62 & 0.05   \\  % 53054-1436-303
122 & J105755.67$+$482502.0 & 0.0733 & 18.20 & 0.53 & 0.07   \\  % 52643-0963-626
123 & J110036.57$+$064121.4 & 0.2993 & 18.90 & 0.55 & 0.10   \\  % 52646-1002-117
124 & J110039.66$+$085927.1 & 0.0626 & 17.12 & 0.71 & 0.11   \\  % 52723-1220-172
125 & J110258.74$+$463811.5 & 0.1490 & 17.80 & 0.46 & 0.04   \\  % 53054-1436-523
126 & J110536.35$+$091805.6 & 0.1770 & 19.47 & 0.49 & 0.09   \\  % 52751-1221-253
127 & J110540.46$+$035309.1 & 0.0995 & 17.52 & 0.57 & 0.22   \\  % 52356-0581-254
128 & J110721.89$+$124810.4 & 0.1761 & 18.58 & 0.34 & 0.05   \\  % 53078-1604-332
129 & J110753.16$-$000717.7 & 0.1120 & 17.80 & 0.69 & 0.20   \\  % 51900-0278-279
130 & J110817.77$+$105443.0 & 0.1715 & 18.64 & 0.72 & 0.08   \\  % 53078-1604-242
131 & J111009.50$+$014802.6 & 0.1009 & 18.40 & 0.53 & 0.14   \\  % 52374-0509-143
132 & J111031.61$+$022043.2 & 0.0795 & 18.08 & 0.66 & 0.14   \\  % 52374-0509-508
133 & J111139.94$+$405816.5 & 0.0775 & 18.45 & 0.81 & 0.07   \\  % 53046-1437-636
134 & J111330.25$+$484241.4 & 0.1105 & 18.03 & 0.53 & 0.06   \\  % 52646-0964-636
135 & J111350.05$+$550338.6 & 0.0707 & 17.07 & 0.68 & 0.04   \\  % 52649-1012-401
136 & J111402.17$+$020851.5 & 0.3079 & 19.69 & 0.49 & 0.14   \\  % 52381-0510-198
137 & J111443.66$+$525834.3 & 0.0792 & 17.15 & 0.50 & 0.05   \\  % 52649-1012-133
138 & J111644.65$+$402635.6 & 0.2021 & 20.37 & 0.62 & 0.05   \\  % 53084-1440-250
139 & J112202.23$+$534253.6 & 0.0891 & 17.52 & 0.36 & 0.06   \\  % 52707-1013-169
140 & J112242.74$+$414355.5 & 0.0447 & 18.51 & 0.76 & 0.07   \\  % 53084-1440-512
141 & J112255.73$+$523825.3 & 0.0339 & 15.92 & 0.75 & 0.05   \\  % 52365-0879-328
142 & J112309.17$+$433134.8 & 0.0792 & 17.96 & 0.45 & 0.08   \\  % 53062-1365-124
143 & J112526.52$+$022039.1 & 0.0486 & 16.73 & 0.75 & 0.12   \\  % 52636-0511-031
144 & J112613.04$+$105102.7 & 0.1130 & 18.49 & 0.65 & 0.15   \\  % 52781-1223-409
145 & J112628.73$+$472453.9 & 0.0333 & 17.27 & 0.70 & 0.07   \\  % 53083-1441-619
146 & J112637.74$+$513423.0 & 0.0264 & 16.02 & 0.67 & 0.04   \\  % 52365-0879-200
147 & J112713.22$+$462530.6 & 0.1060 & 19.68 & 0.91 & 0.06   \\  % 53050-1442-263
148 & J112718.75$+$585025.1 & 0.0878 & 16.91 & 0.76 & 0.06   \\  % 52409-0952-228
149 & J113545.55$+$644005.3 & 0.1132 & 17.79 & 0.57 & 0.04   \\  % 52059-0597-560
150 & J113638.38$+$424553.0 & 0.0711 & 17.56 & 0.64 & 0.09   \\  % 53055-1443-608
151 & J113657.68$+$411318.5 & 0.0717 & 18.26 & 0.47 & 0.08   \\  % 53055-1443-009
152 & J113711.45$+$123951.5 & 0.0800 & 17.10 & 0.67 & 0.12   \\  % 53083-1607-513
153 & J114008.71$+$030711.4 & 0.0811 & 17.33 & 0.51 & 0.08   \\  % 51994-0514-331
154 & J114107.56$-$024910.8 & 0.0287 & 15.61 & 0.67 & 0.11   \\  % 52282-0328-197
155 & J114212.76$+$451037.6 & 0.3293 & 19.32 & 0.30 & 0.08   \\  % 53083-1367-481
156 & J114330.98$+$643248.6 & 0.1235 & 18.29 & 0.27 & 0.10   \\  % 52316-0598-301
157 & J114339.49$-$024316.3 & 0.0935 & 18.26 & 0.60 & 0.08   \\  % 52282-0328-107
158 & J114343.77$+$550019.3 & 0.0271 & 17.48 & 0.34 & 0.04   \\  % 52734-1015-596
159 & J114449.45$+$442300.5 & 0.1659 & 18.60 & 0.50 & 0.08   \\  % 53084-1368-285
160 & J114633.99$+$100245.0 & 0.1243 & 18.72 & 0.63 & 0.14   \\  % 52734-1226-485
161 & J114723.20$-$025004.7 & 0.1213 & 17.80 & 0.56 & 0.10   \\  % 52056-0329-169
162 & J114851.62$+$514528.7 & 0.0676 & 18.51 & 0.71 & 0.07   \\  % 52367-0880-032
163 & J115138.11$+$561331.9 & 0.0509 & 17.25 & 0.58 & 0.03   \\  % 52781-1312-121
164 & J115341.78$+$461242.3 & 0.0244 & 15.14 & 0.64 & 0.11   \\  % 53080-1446-129
165 & J115739.55$+$593414.3 & 0.1705 & 18.92 & 0.58 & 0.07   \\  % 52411-0953-077
166 & J120449.71$+$510043.9 & 0.0826 & 17.55 & 0.49 & 0.07   \\  % 52442-0969-445
167 & J121503.69$-$013210.6 & 0.1081 & 17.83 & 0.65 & 0.09   \\  % 52367-0332-604
168 & J121511.09$+$450945.1 & 0.0551 & 16.72 & 0.71 & 0.05   \\  % 53090-1370-483
169 & J121518.24$+$014751.2 & 0.0709 & 18.00 & 0.61 & 0.10   \\  % 52282-0518-218
170 & J121629.13$+$601823.5 & 0.0602 & 17.88 & 0.70 & 0.06   \\  % 52409-0955-466
171 & J121803.05$+$501728.3 & 0.1923 & 18.71 & 0.64 & 0.07   \\  % 52413-0970-558
172 & J121828.57$+$533137.0 & 0.0635 & 17.03 & 0.74 & 0.09   \\  % 52430-0883-606
173 & J121836.98$+$091323.6 & 0.0775 & 17.71 & 0.59 & 0.07   \\  % 52672-1230-131
174 & J122342.81$+$581446.2 & 0.0145 & 16.09 & 0.63 & 0.05   \\  % 52791-1315-568
175 & J122349.64$+$072657.9 & 0.0747 & 16.99 & 0.79 & 0.08   \\  % 53140-1625-071
176 & J122658.41$+$421835.3 & 0.1388 & 18.13 & 0.63 & 0.13   \\  % 53112-1452-157
177 & J122711.67$+$630646.9 & 0.0779 & 19.26 & 0.47 & 0.05   \\  % 52342-0779-621
178 & J122844.83$+$654234.5 & 0.0891 & 17.84 & 0.59 & 0.07   \\  % 52317-0600-437
179 & J123152.81$+$001033.7 & 0.1916 & 20.67 & 0.74 & 0.09   \\  % 51990-0289-625
180 & J123349.92$+$634957.1 & 0.1334 & 19.15 & 0.64 & 0.05   \\  % 52317-0600-043
181 & J124035.82$-$002919.5 & 0.0809 & 17.99 & 0.47 & 0.10   \\  % 51941-0290-021
182 & J124118.74$+$010040.1 & 0.0899 & 17.85 & 0.54 & 0.06   \\  % 51928-0291-375
183 & J124221.62$+$575304.0 & 0.1047 & 18.26 & 0.57 & 0.04   \\  % 52765-1317-421
184 & J124226.30$+$521028.2 & 0.2350 & 19.27 & 0.23 & 0.06   \\  % 52379-0885-107
185 & J124738.52$+$621243.1 & 0.1210 & 18.74 & 0.38 & 0.05   \\  % 52373-0781-076
186 & J125055.28$-$015556.8 & 0.0814 & 18.23 & 0.37 & 0.09   \\  % 51997-0337-425
187 & J125359.22$+$655907.6 & 0.0935 & 18.29 & 0.63 & 0.10   \\  % 52316-0601-533
188 & J125359.62$+$462750.1 & 0.0617 & 17.90 & 0.76 & 0.06   \\  % 53116-1457-236
189 & J125654.92$+$494054.4 & 0.1730 & 19.86 & 0.60 & 0.05   \\  % 52736-1279-075
190 & J130030.38$+$010247.5 & 0.0676 & 17.09 & 0.67 & 0.10   \\  % 51994-0293-525
191 & J130311.23$-$004532.7 & 0.1889 & 18.61 & 0.49 & 0.07   \\  % 51986-0294-296
192 & J130716.99$+$450645.3 & 0.0840 & 18.51 & 0.76 & 0.06   \\  % 53083-1374-542
193 & J130803.88$+$505226.7 & 0.0542 & 17.65 & 0.70 & 0.04   \\  % 52376-0887-100
194 & J131009.44$+$023343.7 & 0.2167 & 19.18 & 0.42 & 0.11   \\  % 52027-0524-640
195 & J131303.47$+$633235.2 & 0.1930 & 18.31 & 0.68 & 0.06   \\  % 52072-0602-051
196 & J131305.81$+$012755.9 & 0.0294 & 16.03 & 0.77 & 0.17   \\  % 52295-0525-091
197 & J131310.13$+$051942.2 & 0.0487 & 17.51 & 0.66 & 0.15   \\  % 52338-0850-585
198 & J131533.29$+$122200.5 & 0.1464 & 18.02 & 0.66 & 0.11   \\  % 53142-1697-464
199 & J131537.07$+$151955.3 & 0.1245 & 19.00 & 0.46 & 0.11   \\  % 53112-1773-411
200 & J131558.14$+$135414.6 & 0.1520 & 19.08 & 0.45 & 0.08   \\  % 53112-1773-226
201 & J131618.85$+$021407.5 & 0.0723 & 17.57 & 0.59 & 0.10   \\  % 52312-0526-309
202 & J131715.12$+$484630.3 & 0.1311 & 18.77 & 0.75 & 0.04   \\  % 52759-1282-271
203 & J131804.32$+$411734.6 & 0.0674 & 15.95 & 0.55 & 0.06   \\  % 53138-1460-004
204 & J131926.53$+$105611.0 & 0.0643 & 17.29 & 0.52 & 0.09   \\  % 53146-1698-257
205 & J132224.41$+$422643.4 & 0.0741 & 17.90 & 0.56 & 0.05   \\  % 53089-1376-087
206 & J132428.24$+$044629.7 & 0.0214 & 16.21 & 0.73 & 0.11   \\  % 52375-0852-394
207 & J132711.09$+$653618.1 & 0.1146 & 18.91 & 0.42 & 0.07   \\  % 51988-0496-091
208 & J132834.37$-$030744.8 & 0.0852 & 17.70 & 0.81 & 0.15   \\  % 52426-0911-283
209 & J132953.44$-$025523.4 & 0.1835 & 18.74 & 0.51 & 0.15   \\  % 52377-0910-144
210 & J133704.91$+$022050.2 & 0.1130 & 18.13 & 0.73 & 0.09   \\  % 52022-0528-152
211 & J133921.95$+$544527.7 & 0.1012 & 19.71 & 0.54 & 0.04   \\  % 52764-1321-044
212 & J133928.50$+$403229.9 & 0.1179 & 18.29 & 0.53 & 0.02   \\  % 53091-1464-029
213 & J134144.52$-$005832.8 & 0.1475 & 18.46 & 0.54 & 0.11   \\  % 51671-0299-134
214 & J134249.27$+$482723.7 & 0.0912 & 17.53 & 0.40 & 0.04   \\  % 52762-1283-635
215 & J134516.78$-$011054.8 & 0.1465 & 19.45 & 0.63 & 0.12   \\  % 51943-0300-281
216 & J134632.14$+$642325.1 & 0.0241 & 15.80 & 0.55 & 0.09   \\  % 52079-0604-536
217 & J134738.24$+$474301.9 & 0.0641 & 16.72 & 0.42 & 0.08   \\  % 52736-1284-151
218 & J134814.89$+$021316.3 & 0.0683 & 17.94 & 0.44 & 0.10   \\  % 52026-0530-183
219 & J135159.16$+$025034.0 & 0.0734 & 17.66 & 0.68 & 0.11   \\  % 52026-0530-541
220 & J135724.00$+$654116.6 & 0.1421 & 19.12 & 0.68 & 0.07   \\  % 51984-0498-344
221 & J135724.51$+$652505.9 & 0.1063 & 18.46 & 0.37 & 0.08   \\  % 51989-0497-014
222 & J140040.57$-$015518.3 & 0.0250 & 16.06 & 0.53 & 0.25   \\  % 52443-0915-437
223 & J140630.10$-$001939.6 & 0.1062 & 20.27 & 0.69 & 0.17   \\  % 51688-0302-227
224 & J140702.44$+$135537.7 & 0.1344 & 18.65 & 0.80 & 0.09   \\  % 53178-1704-481
225 & J141234.67$-$003500.1 & 0.1270 & 18.20 & 0.59 & 0.18   \\  % 51615-0303-302
226 & J141325.86$+$434101.3 & 0.1667 & 18.27 & 0.59 & 0.03   \\  % 53108-1394-391
227 & J141435.58$+$003312.6 & 0.1809 & 18.48 & 0.63 & 0.14   \\  % 51615-0303-435
228 & J141515.40$+$043616.0 & 0.0553 & 18.46 & 0.86 & 0.11   \\  % 52055-0583-174
229 & J141849.66$+$464943.4 & 0.1379 & 18.51 & 0.64 & 0.04   \\  % 52728-1287-365
230 & J142119.13$+$631300.2 & 0.1344 & 19.28 & 0.69 & 0.06   \\  % 51988-0499-293
231 & J142145.61$+$621713.8 & 0.1052 & 17.99 & 0.61 & 0.07   \\  % 52365-0606-565
232 & J142449.48$+$012353.6 & 0.1076 & 18.65 & 0.45 & 0.11   \\  % 51997-0534-047
233 & J142543.21$+$344952.9 & 0.1786 & 19.45 & 0.59 & 0.06   \\  % 53144-1644-094
234 & J142732.21$+$343039.1 & 0.0686 & 16.37 & 0.63 & 0.06   \\  % 53144-1644-048
235 & J143010.84$+$572202.1 & 0.1113 & 18.36 & 0.78 & 0.03   \\  % 52441-0790-230
236 & J143047.53$+$565729.1 & 0.0922 & 17.90 & 0.75 & 0.04   \\  % 52441-0790-253
237 & J143114.31$+$452705.9 & 0.1248 & 18.57 & 0.52 & 0.05   \\  % 52731-1288-430
238 & J143310.55$+$525830.5 & 0.0474 & 17.69 & 0.84 & 0.03   \\  % 52781-1327-377
239 & J143450.63$+$033842.6 & 0.0282 & 15.62 & 0.63 & 0.15   \\  % 52023-0586-234
240 & J143451.39$-$022439.8 & 0.1507 & 18.22 & 0.64 & 0.20   \\  % 52409-0919-223
241 & J143544.50$+$572427.9 & 0.2204 & 19.28 & 0.37 & 0.04   \\  % 52441-0790-156
242 & J143552.31$+$341345.5 & 0.0450 & 18.15 & 0.67 & 0.06   \\  % 53172-1645-139
243 & J143710.11$-$014054.5 & 0.0566 & 16.79 & 0.65 & 0.15   \\  % 52409-0919-512
244 & J143713.55$+$545818.7 & 0.0933 & 17.76 & 0.65 & 0.05   \\  % 52668-1162-156
245 & J144052.61$-$023506.3 & 0.0443 & 16.31 & 0.53 & 0.23   \\  % 52411-0920-289
246 & J144108.70$+$351958.8 & 0.0792 & 17.13 & 0.49 & 0.03   \\  % 53172-1645-626
247 & J144249.72$+$611137.8 & 0.0479 & 18.22 & 0.73 & 0.09   \\  % 52081-0608-405
248 & J144705.47$+$003653.2 & 0.0955 & 19.57 & 0.60 & 0.18   \\  % 51662-0308-492
249 & J144855.61$+$571039.0 & 0.1052 & 18.02 & 0.53 & 0.06   \\  % 52435-0791-511
250 & J145751.91$+$000011.5 & 0.1872 & 19.28 & 0.62 & 0.21   \\  % 51994-0309-071
251 & J150224.73$+$452353.9 & 0.0680 & 16.92 & 0.63 & 0.09   \\  % 53147-1676-530
252 & J150648.86$+$341306.8 & 0.0882 & 16.68 & 0.40 & 0.06   \\  % 53108-1385-233
253 & J150752.53$+$515111.1 & 0.0748 & 17.22 & 0.67 & 0.08   \\  % 52703-1165-424
254 & J150835.15$-$013106.3 & 0.0708 & 18.03 & 0.61 & 0.26   \\  % 52426-0922-589
255 & J151257.19$+$031136.4 & 0.2222 & 19.20 & 0.69 & 0.15   \\  % 52057-0590-103
256 & J151928.18$+$333628.1 & 0.0816 & 17.41 & 0.47 & 0.08   \\  % 53116-1386-550
257 & J152205.41$+$393441.3 & 0.0766 & 16.31 & 0.86 & 0.09   \\  % 52765-1293-387
258 & J152325.78$+$395902.3 & 0.1035 & 17.60 & 0.63 & 0.08   \\  % 52736-1292-026
259 & J152347.00$+$541720.4 & 0.1594 & 18.08 & 0.73 & 0.05   \\  % 52376-0794-550
260 & J153001.82$-$020415.1 & 0.0512 & 17.15 & 0.69 & 0.58   \\  % 52411-0925-266
261 & J153425.59$+$040806.7 & 0.0395 & 18.66 & 0.56 & 0.17   \\  % 52026-0593-547
262 & J153656.44$+$312248.1 & 0.0562 & 17.61 & 0.01 & 0.08   \\  % 53119-1388-039
263 & J154150.86$+$310037.2 & 0.0686 & 16.28 & 0.60 & 0.11   \\  % 53135-1389-611
264 & J154257.49$+$030653.3 & 0.0656 & 17.82 & 0.64 & 0.23   \\  % 52045-0594-216
265 & J154623.62$+$475122.2 & 0.1033 & 18.37 & 0.58 & 0.05   \\  % 52731-1168-417
266 & J154639.95$+$442930.0 & 0.1308 & 19.71 & 0.61 & 0.06   \\  % 52782-1333-153
267 & J155711.97$+$390928.9 & 0.0982 & 17.71 & 0.63 & 0.05   \\  % 52516-1054-128
268 & J160656.04$+$371917.8 & 0.0411 & 16.09 & 0.56 & 0.05   \\  % 52761-1055-086
269 & J161227.84$+$010159.9 & 0.0971 & 18.58 & 0.52 & 0.42   \\  % 51690-0345-601
270 & J161751.99$-$001957.4 & 0.0569 & 17.26 & 0.63 & 0.38   \\  % 51693-0346-147
271 & J161809.38$+$361957.8 & 0.0340 & 16.41 & 0.56 & 0.05   \\  % 52764-1056-067
272 & J161927.81$+$395832.3 & 0.0324 & 15.90 & 0.80 & 0.03   \\  % 52759-1172-346
273 & J162021.15$+$301020.5 & 0.0964 & 17.38 & 0.57 & 0.11   \\  % 53146-1420-093
274 & J162403.64$-$005410.4 & 0.0464 & 16.32 & 0.74 & 0.38   \\  % 52000-0364-259
275 & J162542.16$-$004330.2 & 0.1217 & 19.02 & 0.67 & 0.34   \\  % 52000-0364-128
276 & J162636.40$+$350242.1 & 0.0340 & 15.73 & 0.46 & 0.08   \\  % 52522-1057-630
277 & J162824.49$+$452811.0 & 0.2279 & 19.31 & 0.59 & 0.02   \\  % 52057-0626-433
278 & J163159.59$+$243740.3 & 0.0435 & 17.67 & 0.60 & 0.18   \\  % 53177-1572-457
279 & J163843.84$+$473051.7 & 0.1792 & 19.81 & 0.45 & 0.08   \\  % 52144-0627-631
280 & J164027.63$+$471256.5 & 0.1097 & 17.87 & 0.66 & 0.08   \\  % 52144-0627-604
281 & J164902.89$+$223959.5 & 0.1042 & 21.33 & 0.15 & 0.22   \\  % 52912-1424-260
282 & J164907.63$+$642422.3 & 0.1835 & 18.87 & 0.63 & 0.14   \\  % 51699-0349-364
283 & J170812.29$+$601512.7 & 0.1445 & 18.15 & 0.76 & 0.08   \\  % 51703-0353-460
284 & J170902.07$+$641728.1 & 0.0894 & 19.39 & 0.42 & 0.11   \\  % 51691-0350-263
285 & J171457.68$+$544455.0 & 0.1414 & 19.36 & 0.63 & 0.07   \\  % 51997-0367-298
286 & J172037.15$+$574856.3 & 0.1327 & 19.38 & 0.69 & 0.09   \\  % 51788-0355-585
287 & J172759.14$+$542147.1 & 0.0995 & 19.27 & 0.58 & 0.15   \\  % 51821-0359-535
288 & J205000.01$+$003124.8 & 0.1638 & 19.25 & 0.59 & 0.34   \\  % 52443-0983-382
289 & J205822.14$-$065004.4 & 0.0738 & 18.35 & 0.38 & 0.22   \\  % 52176-0636-105
290 & J210226.54$+$000702.3 & 0.0516 & 17.67 & 0.70 & 0.28   \\  % 52431-0985-396
291 & J211145.90$+$093813.7 & 0.1391 & 18.87 & 0.99 & 0.39   \\  % 52520-0728-179
292 & J211438.55$+$111321.2 & 0.0844 & 18.84 & 0.90 & 0.35   \\  % 52520-0728-563
293 & J212329.42$-$081255.0 & 0.1169 & 19.35 & 0.68 & 0.32   \\  % 52178-0640-252
294 & J213418.32$-$064335.3 & 0.0517 & 18.08 & 0.72 & 0.14   \\  % 52199-0641-531
295 & J221139.16$-$010535.1 & 0.0926 & 17.33 & 0.66 & 0.37   \\  % 51791-0374-287
296 & J221458.23$-$082020.6 & 0.1236 & 18.73 & 0.66 & 0.23   \\  % 52206-0718-608
297 & J223811.33$+$143343.4 & 0.1566 & 18.71 & 0.53 & 0.29   \\  % 52520-0739-416
298 & J225630.07$+$141020.7 & 0.1509 & 19.46 & 0.57 & 0.18   \\  % 52263-0742-353
299 & J230649.78$+$005023.4 & 0.0607 & 17.30 & 0.71 & 0.21   \\  % 51811-0381-363
300 & J230920.84$+$150134.8 & 0.0995 & 18.48 & 1.09 & 1.08   \\  % 52262-0743-506
301 & J230942.43$-$103529.5 & 0.2381 & 20.73 & 0.58 & 0.12   \\  % 52226-0726-257
302 & J233108.07$-$094711.8 & 0.2529 & 19.42 & 0.44 & 0.10   \\  % 52523-0646-560
303 & J233837.09$-$002810.5 & 0.0356 & 16.88 & 0.61 & 0.12   \\  % 51877-0385-264
304 & J233853.83$+$004812.5 & 0.1697 & 18.73 & 0.54 & 0.14   \\  % 51877-0385-379
305 & J234143.38$-$005518.6 & 0.0813 & 17.46 & 0.74 & 0.11   \\  % 51877-0385-121
306 & J234807.14$-$091202.6 & 0.0777 & 18.49 & 0.68 & 0.13   \\  % 52559-0648-572
307 & J235059.66$+$145706.3 & 0.1349 & 18.57 & 0.67 & 0.13   \\  % 52226-0749-439
308 & J235129.98$+$000403.7 & 0.0992 & 18.14 & 0.70 & 0.14   \\  % 51788-0386-197
309 & J235833.21$+$003453.5 & 0.0756 & 17.49 & 0.55 & 0.12   \\  % 51791-0387-432


==> full_table2.tex <==
%%ID&   LOGF_3727  &   LOGF_4570  &   LOGF_NHB  &   LOGF_BHB  &    LOGF_5007  &   LOGF_6300  &   LOGF_NHA  &    LOGF_BHA  &   LOGF_6583  &   LOGF_6716  &   LOGF_6731  &  FWHM_BHA  &  FWHM_OIII  &  FWHM_SII      %  SPEC
1   &    $-$15.12  &   $<-$15.45  &   $-$15.39  &  $<-$15.76  &     $-$14.79  &    $-$15.84  &   $-$14.65  &    $-$14.71  &    $-$15.08  &    $-$15.28  &    $-$15.46  &      1921  &        215  &       195  \\  %  52143-0650-174
2   &    $-$15.32  &    $-$15.19  &   $-$15.61  &   $-$15.34  &     $-$15.44  &    $-$16.11  &   $-$15.08  &    $-$14.78  &    $-$15.51  &    $-$15.74  &    $-$15.87  &       924  &        164  &       158  \\  %  52235-0750-609
3   &    $-$15.34  &   $<-$15.38  &   $-$15.40  &  $<-$15.81  &     $-$15.13  &    $-$16.12  &   $-$14.74  &    $-$14.62  &    $-$14.95  &    $-$15.49  &    $-$15.53  &      1022  &        168  &       256  \\  %  51795-0389-120
4   &    $-$15.77  &   $<-$15.56  &   $-$15.97  &   $-$15.46  &     $-$15.43  &    $-$16.19  &   $-$15.29  &    $-$14.87  &    $-$15.38  &    $-$15.84  &    $-$16.02  &      1108  &        305  &       289  \\  %  51900-0390-624
5   &    $-$15.44  &   $<-$15.41  &   $-$15.75  &    \nodata  &     $-$15.05  &    $-$15.86  &   $-$15.00  &    $-$14.84  &    $-$15.10  &    $-$15.54  &    $-$15.64  &      1407  &        279  &       290  \\  %  51821-0417-182
6   &    $-$14.91  &   $<-$15.29  &   $-$15.66  &   $-$15.10  &     $-$15.26  &    $-$15.80  &   $-$15.05  &    $-$14.70  &    $-$15.75  &    $-$15.52  &    $-$15.65  &      2235  &        146  &       176  \\  %  52162-0655-089
7   &    $-$15.08  &   $<-$15.69  &   $-$15.46  &   $-$15.18  &     $-$14.75  &    $-$15.91  &   $-$14.88  &    $-$14.68  &    $-$15.18  &    $-$15.59  &    $-$15.72  &       824  &        182  &       192  \\  %  51913-0394-624
8   &    $-$15.31  &   $<-$15.43  &   $-$15.69  &   $-$15.24  &     $-$15.22  &    $-$16.25  &   $-$15.06  &    $-$14.75  &    $-$15.43  &    $-$15.76  &    $-$15.83  &      1187  &        395  &       148  \\  %  52146-0658-488
9   &    $-$14.85  &    $-$14.79  &   $-$15.18  &   $-$14.83  &     $-$14.75  &    $-$15.91  &   $-$14.60  &    $-$14.33  &    $-$15.10  &    $-$15.41  &    $-$15.55  &       678  &        229  &       104  \\  %  51811-0422-321
10  &    $-$15.49  &    $-$14.65  &   $-$15.75  &   $-$14.36  &     $-$14.55  &    $-$16.03  &   $-$15.00  &    $-$13.91  &    $-$15.42  &    $-$15.77  &    $-$15.82  &       947  &        210  &       133  \\  %  51811-0422-224
11  &    $-$14.97  &    $-$15.12  &   $-$15.28  &   $-$14.97  &     $-$14.58  &    $-$15.84  &   $-$14.76  &    $-$14.36  &    $-$15.24  &    $-$15.44  &    $-$15.56  &       607  &        157  &       182  \\  %  52177-0660-142
12  &    $-$15.48  &    $-$15.36  &   $-$15.58  &   $-$15.31  &     $-$15.37  &   $<-$16.12  &   $-$15.13  &    $-$14.68  &    $-$15.32  &    $-$15.76  &    $-$15.94  &      1204  &        336  &       291  \\  %  51817-0399-317
13  &    $-$15.24  &   $<-$15.37  &   $-$15.44  &   $-$15.10  &     $-$15.04  &    $-$16.01  &   $-$14.84  &    $-$14.48  &    $-$15.20  &    $-$15.47  &    $-$15.63  &      1342  &        243  &       236  \\  %  52163-0661-229
14  &    $-$15.08  &    $-$14.59  &   $-$15.61  &   $-$14.64  &     $-$14.78  &   $<-$15.87  &   $-$15.11  &    $-$14.12  &    $-$14.85  &    $-$15.35  &    $-$15.40  &       731  &        454  &       358  \\  %  51893-0424-097
15  &    $-$15.37  &    $-$14.88  &   $-$15.53  &   $-$15.01  &     $-$15.01  &    $-$15.97  &   $-$14.99  &    $-$14.52  &    $-$15.14  &    $-$15.73  &    $-$15.87  &       706  &        185  &       227  \\  %  51820-0429-084
16  &    $-$15.50  &   $<-$15.49  &   $-$15.90  &   $-$15.39  &     $-$15.36  &    $-$16.27  &   $-$15.14  &    $-$15.05  &    $-$15.57  &    $-$15.94  &    $-$16.03  &      2085  &        132  &       149  \\  %  51900-0427-492
17  &    $-$15.25  &    $-$15.00  &   $-$15.65  &   $-$14.71  &     $-$14.86  &    $-$15.98  &   $-$14.98  &    $-$14.19  &    $-$15.32  &    $-$15.58  &    $-$15.66  &       909  &        277  &       129  \\  %  51820-0407-329
18  &    $-$15.26  &   $<-$15.59  &   $-$15.43  &   $-$15.21  &     $-$15.00  &    $-$16.25  &   $-$14.80  &    $-$14.67  &    $-$15.28  &    $-$15.66  &    $-$15.77  &       688  &        185  &       201  \\  %  51908-0454-109
19  &    $-$15.16  &    $-$15.06  &   $-$15.24  &   $-$14.77  &     $-$14.92  &    $-$16.10  &   $-$14.55  &    $-$14.30  &    $-$14.83  &    $-$15.32  &    $-$15.48  &       960  &        188  &       135  \\  %  51910-0456-257
20  &    $-$15.08  &   $<-$15.26  &   $-$15.85  &   $-$14.73  &     $-$14.56  &    $-$15.89  &   $-$15.01  &    $-$14.31  &    $-$15.31  &    $-$15.55  &    $-$15.58  &       858  &        176  &       164  \\  %  51910-0456-077
21  &    $-$14.73  &    $-$14.00  &   $-$15.35  &   $-$13.95  &     $-$14.17  &    $-$15.38  &   $-$14.55  &    $-$13.44  &    $-$14.60  &    $-$15.00  &    $-$15.07  &      1088  &        201  &       249  \\  %  51817-0411-513
22  &    $-$14.67  &   $<-$15.18  &   $-$14.97  &   $-$15.24  &     $-$14.74  &    $-$15.83  &   $-$14.38  &    $-$14.33  &    $-$14.72  &    $-$15.19  &    $-$15.28  &      1141  &        195  &       192  \\  %  51929-0413-470
23  &    $-$15.12  &   $<-$15.39  &   $-$15.82  &   $-$14.90  &     $-$14.69  &    $-$16.15  &   $-$15.43  &    $-$14.27  &    $-$15.91  &    $-$15.83  &    $-$16.00  &       828  &        130  &       151  \\  %  51901-0414-405
24  &    $-$15.33  &    $-$14.25  &   $-$14.93  &   $-$14.47  &     $-$14.66  &    $-$15.94  &   $-$14.25  &    $-$13.89  &    $-$14.83  &    $-$15.41  &    $-$15.46  &       930  &        544  &       385  \\  %  51901-0414-426
25  &    $-$15.25  &   $<-$15.40  &   $-$15.39  &  $<-$15.73  &     $-$15.56  &   $<-$16.00  &   $-$14.90  &    $-$15.23  &    $-$15.31  &    $-$15.59  &    $-$15.70  &      1189  &        188  &       203  \\  %  51924-0460-014
26  &    $-$15.53  &    $-$14.59  &   $-$15.74  &   $-$14.71  &     $-$14.95  &    $-$16.09  &   $-$14.91  &    $-$14.11  &    $-$15.10  &    $-$15.67  &    $-$15.90  &       804  &        280  &       153  \\  %  51909-0462-504
27  &    $-$15.23  &    $-$14.46  &   $-$15.89  &   $-$14.42  &     $-$14.30  &    $-$15.31  &   $-$15.27  &    $-$13.83  &    $-$14.88  &    $-$15.37  &    $-$15.41  &      1057  &        351  &       272  \\  %  53034-1734-137
28  &    $-$15.25  &   $<-$15.38  &   $-$15.52  &   $-$15.12  &     $-$15.23  &    $-$15.75  &   $-$14.79  &    $-$14.35  &    $-$15.02  &    $-$15.37  &    $-$15.50  &      1341  &        268  &       207  \\  %  51877-0431-533
29  &    $-$15.11  &   $<-$15.39  &   $-$15.62  &  $<-$15.75  &     $-$15.39  &    $-$16.06  &   $-$15.16  &    $-$14.74  &    $-$15.44  &    $-$15.58  &    $-$15.79  &      1553  &        395  &       137  \\  %  51884-0432-384
30  &    $-$15.42  &   $<-$15.69  &   $-$15.79  &   $-$15.16  &     $-$14.25  &    $-$15.57  &   $-$15.26  &    $-$14.51  &    $-$15.35  &    $-$15.74  &    $-$15.80  &       925  &        594  &       288  \\  %  51959-0541-617
31  &    $-$15.63  &   $<-$15.36  &   $-$15.70  &   $-$15.71  &     $-$15.79  &    $-$16.18  &   $-$15.09  &    $-$15.21  &    $-$15.49  &    $-$15.95  &    $-$16.02  &      1214  &    \nodata  &       101  \\  %  52314-0857-039
32  &    $-$15.32  &   $<-$15.51  &   $-$15.63  &   $-$14.96  &     $-$15.00  &    $-$16.09  &   $-$15.01  &    $-$14.39  &    $-$15.16  &    $-$15.61  &    $-$15.64  &      1622  &        224  &       232  \\  %  51959-0541-602
33  &    $-$14.97  &    $-$14.62  &   $-$15.03  &   $-$14.55  &     $-$14.74  &    $-$15.74  &   $-$14.39  &    $-$13.96  &    $-$14.70  &    $-$15.19  &    $-$15.37  &      1231  &        230  &       261  \\  %  53052-1736-062
34  &    $-$15.63  &   $<-$15.47  &   $-$15.57  &    \nodata  &     $-$15.79  &    $-$15.90  &   $-$14.92  &    $-$15.14  &    $-$15.34  &    $-$15.84  &    $-$15.89  &      1607  &    \nodata  &       253  \\  %  53055-1737-220
35  &    $-$15.33  &    $-$14.91  &   $-$15.56  &   $-$14.66  &     $-$14.60  &    $-$15.95  &   $-$15.00  &    $-$14.06  &    $-$16.12  &    $-$16.00  &   $<-$16.24  &      1170  &        117  &   \nodata  \\  %  53055-1737-468
36  &    $-$14.66  &   $<-$15.40  &   $-$15.12  &   $-$14.99  &     $-$13.71  &    $-$15.18  &   $-$14.59  &    $-$14.36  &    $-$14.62  &    $-$15.09  &    $-$15.00  &       858  &        343  &       274  \\  %  52316-0858-438
37  &    $-$15.34  &    $-$15.37  &   $-$15.72  &   $-$15.36  &     $-$14.92  &    $-$15.73  &   $-$15.16  &    $-$14.69  &    $-$15.26  &    $-$15.69  &    $-$15.68  &      1522  &        347  &       187  \\  %  52583-0890-400
38  &    $-$15.47  &   $<-$15.37  &   $-$15.78  &   $-$15.19  &     $-$15.52  &   $<-$15.92  &   $-$15.00  &    $-$14.61  &    $-$15.31  &    $-$15.65  &    $-$15.87  &      1506  &        487  &       211  \\  %  51869-0437-274
39  &    $-$14.67  &   $<-$15.29  &   $-$14.89  &  $<-$15.69  &     $-$15.10  &    $-$15.91  &   $-$14.32  &    $-$14.72  &    $-$14.59  &    $-$15.20  &    $-$15.27  &      1053  &        112  &        76  \\  %  53090-1780-369
40  &    $-$14.94  &   $<-$15.25  &   $-$15.04  &   $-$15.21  &     $-$14.77  &    $-$15.86  &   $-$14.38  &    $-$14.54  &    $-$14.75  &    $-$15.18  &    $-$15.33  &      1394  &        141  &       165  \\  %  52670-1205-330
41  &    $-$15.77  &    $-$14.33  &   $-$15.65  &   $-$14.39  &     $-$15.08  &    $-$16.27  &  $<-$15.65  &    $-$13.82  &    $-$15.70  &    $-$16.08  &    $-$16.11  &       903  &        344  &       111  \\  %  53080-1756-305
42  &    $-$15.52  &   $<-$15.35  &   $-$15.44  &   $-$15.51  &     $-$15.55  &   $<-$16.09  &   $-$14.79  &    $-$14.77  &    $-$15.22  &    $-$15.75  &    $-$15.97  &      1328  &        167  &       131  \\  %  52253-0758-109
43  &    $-$15.20  &    $-$15.22  &   $-$15.58  &   $-$14.76  &     $-$15.15  &   $<-$15.94  &   $-$14.95  &    $-$14.12  &    $-$15.30  &    $-$15.70  &    $-$15.72  &       957  &        247  &       121  \\  %  52705-1265-139
44  &    $-$15.14  &   $<-$15.35  &   $-$15.20  &  $<-$15.53  &     $-$15.11  &   $<-$16.01  &   $-$14.65  &    $-$14.74  &    $-$14.90  &    $-$15.42  &    $-$15.58  &      1193  &        222  &       261  \\  %  52378-0892-244
45  &    $-$14.82  &   $<-$15.35  &   $-$15.06  &   $-$14.81  &     $-$14.68  &    $-$15.74  &   $-$14.49  &    $-$14.25  &    $-$14.80  &    $-$15.14  &    $-$15.31  &       964  &        170  &       178  \\  %  51877-0439-216
46  &    $-$14.67  &   $<-$15.29  &   $-$15.09  &   $-$15.35  &     $-$14.04  &    $-$15.30  &   $-$14.54  &    $-$14.55  &    $-$14.86  &    $-$15.08  &    $-$15.11  &      1346  &        258  &       243  \\  %  52318-0861-430
47  &    $-$15.26  &    $-$15.04  &   $-$15.89  &   $-$14.91  &     $-$14.65  &    $-$15.82  &   $-$15.31  &    $-$14.36  &    $-$15.47  &    $-$15.74  &    $-$15.90  &       823  &        293  &       183  \\  %  52325-0862-287
48  &    $-$15.06  &   $<-$15.26  &   $-$15.20  &   $-$15.32  &     $-$15.06  &    $-$15.89  &   $-$14.60  &    $-$14.69  &    $-$15.10  &    $-$15.42  &    $-$15.50  &      1177  &        182  &       180  \\  %  52709-1266-109
49  &    $-$15.33  &   $<-$15.35  &   $-$15.56  &    \nodata  &     $-$15.11  &    $-$15.75  &   $-$14.96  &    $-$14.99  &    $-$15.16  &    $-$15.60  &    $-$15.71  &      1699  &        347  &       195  \\  %  51868-0441-438
50  &    $-$15.70  &   $<-$15.39  &   $-$15.82  &   $-$15.68  &     $-$15.40  &   $<-$16.00  &   $-$15.11  &    $-$15.04  &    $-$15.40  &    $-$16.03  &    $-$16.06  &       948  &        246  &       202  \\  %  51868-0441-106
51  &    $-$15.69  &    $-$14.63  &  $<-$15.94  &   $-$14.64  &     $-$15.09  &   $<-$15.72  &   $-$15.15  &    $-$14.23  &    $-$15.58  &    $-$16.24  &   $<-$15.97  &      1092  &        146  &   \nodata  \\  %  52962-1585-549
52  &    $-$15.65  &   $<-$15.42  &   $-$15.84  &   $-$15.92  &     $-$14.92  &    $-$15.75  &   $-$15.29  &    $-$15.11  &    $-$15.44  &    $-$15.83  &    $-$15.95  &      1486  &        332  &       160  \\  %  52962-1296-371
53  &    $-$14.71  &   $<-$15.40  &   $-$15.36  &   $-$14.78  &     $-$14.55  &    $-$15.69  &   $-$14.83  &    $-$14.13  &    $-$14.80  &    $-$15.11  &    $-$15.19  &       740  &        359  &       257  \\  %  51882-0442-420
54  &    $-$14.65  &    $-$15.05  &   $-$14.74  &   $-$14.60  &     $-$14.78  &    $-$15.69  &   $-$14.15  &    $-$14.05  &    $-$14.56  &    $-$14.94  &    $-$15.08  &       911  &        213  &       224  \\  %  52589-0893-636
55  &    $-$14.94  &   $<-$15.45  &   $-$15.41  &   $-$15.51  &     $-$15.22  &    $-$15.43  &   $-$14.84  &    $-$14.70  &    $-$15.28  &    $-$15.32  &    $-$15.42  &      1305  &        381  &       311  \\  %  53084-1758-332
56  &    $-$15.20  &    $-$15.20  &   $-$15.36  &   $-$15.46  &     $-$15.52  &   $<-$16.17  &   $-$14.85  &    $-$14.72  &    $-$15.45  &    $-$15.61  &    $-$15.80  &       531  &        150  &       101  \\  %  52932-1267-107
57  &    $-$14.37  &    $-$14.72  &   $-$14.66  &   $-$14.12  &     $-$13.79  &    $-$15.29  &   $-$14.11  &    $-$13.62  &    $-$14.53  &    $-$14.86  &    $-$14.93  &       871  &        198  &       188  \\  %  51873-0443-514
58  &    $-$16.09  &   $<-$15.45  &   $-$16.03  &  $<-$15.72  &     $-$15.31  &    $-$16.33  &   $-$15.45  &    $-$15.12  &    $-$15.71  &    $-$16.08  &    $-$16.08  &      1767  &        220  &       162  \\  %  53084-1758-524
59  &    $-$15.13  &   $<-$15.46  &   $-$15.46  &   $-$15.62  &     $-$15.36  &   $<-$16.02  &   $-$14.88  &    $-$14.82  &    $-$15.23  &    $-$15.54  &    $-$15.82  &       718  &        292  &       283  \\  %  51873-0445-301
60  &    $-$14.88  &   $<-$15.45  &   $-$15.15  &   $-$15.41  &     $-$15.08  &    $-$15.85  &   $-$14.53  &    $-$14.69  &    $-$14.96  &    $-$15.26  &    $-$15.45  &       847  &        172  &       113  \\  %  52963-1297-154
61  &    $-$14.80  &   $<-$15.38  &   $-$15.24  &   $-$15.53  &     $-$15.33  &    $-$15.13  &   $-$14.58  &    $-$14.67  &    $-$15.43  &    $-$15.08  &    $-$15.12  &      2094  &        426  &       450  \\  %  51899-0446-271
62  &    $-$15.09  &    $-$14.39  &   $-$14.78  &   $-$14.59  &     $-$14.92  &    $-$15.97  &   $-$14.23  &    $-$14.05  &    $-$14.93  &    $-$15.40  &    $-$15.60  &       959  &        306  &       261  \\  %  53081-1759-148
63  &    $-$15.59  &   $<-$15.45  &   $-$15.56  &   $-$15.49  &     $-$15.17  &   $<-$16.22  &   $-$14.93  &    $-$14.57  &    $-$15.17  &    $-$15.57  &    $-$15.85  &       837  &        326  &       301  \\  %  52964-1298-335
64  &    $-$15.63  &   $<-$15.48  &   $-$16.04  &  $<-$15.85  &     $-$15.89  &    $-$16.34  &   $-$15.31  &    $-$15.29  &    $-$15.67  &    $-$16.01  &    $-$15.87  &      1369  &    \nodata  &       136  \\  %  52320-0864-067
65  &    $-$14.49  &    $-$14.32  &   $-$14.96  &   $-$14.26  &     $-$13.83  &    $-$15.41  &   $-$14.35  &    $-$13.72  &    $-$14.61  &    $-$15.09  &    $-$15.10  &       721  &        278  &       393  \\  %  52323-0865-191
66  &    $-$15.31  &   $<-$15.34  &   $-$15.60  &   $-$15.74  &     $-$14.89  &   $<-$16.09  &   $-$14.93  &    $-$14.53  &    $-$15.20  &    $-$15.61  &    $-$15.70  &      1223  &        293  &       165  \\  %  52672-0934-517
67  &    $-$15.12  &    $-$14.68  &   $-$15.56  &   $-$14.67  &     $-$14.59  &    $-$15.76  &   $-$14.92  &    $-$14.25  &    $-$15.03  &    $-$15.44  &    $-$15.56  &       847  &        185  &       158  \\  %  51877-0447-554
68  &    $-$15.25  &    $-$15.19  &   $-$15.59  &   $-$14.78  &     $-$15.29  &    $-$16.24  &   $-$14.93  &    $-$14.26  &    $-$15.06  &    $-$15.65  &    $-$15.69  &      1093  &        162  &       176  \\  %  52293-0830-239
69  &    $-$15.38  &    $-$14.78  &   $-$15.51  &   $-$14.94  &     $-$15.25  &    $-$15.84  &   $-$14.82  &    $-$14.40  &    $-$15.01  &    $-$15.59  &    $-$15.59  &       767  &        229  &       310  \\  %  52605-0897-178
70  &    $-$15.79  &    $-$14.20  &   $-$15.58  &   $-$14.55  &     $-$15.16  &   $<-$16.03  &   $-$14.77  &    $-$14.16  &    $-$15.28  &    $-$15.87  &    $-$15.92  &       800  &        427  &       245  \\  %  52964-1211-420
71  &    $-$15.52  &   $<-$15.55  &   $-$15.72  &   $-$15.53  &     $-$15.32  &    $-$16.36  &   $-$14.94  &    $-$15.02  &    $-$15.20  &    $-$15.71  &    $-$15.81  &       582  &        277  &       149  \\  %  51900-0449-571
72  &    $-$15.07  &   $<-$15.43  &   $-$15.65  &   $-$15.55  &     $-$14.80  &    $-$15.83  &   $-$15.11  &    $-$14.83  &    $-$15.16  &    $-$15.51  &    $-$15.67  &      1784  &        314  &       214  \\  %  52294-0831-464
73  &    $-$14.83  &    $-$14.45  &   $-$14.81  &   $-$14.08  &     $-$14.08  &    $-$15.62  &   $-$14.22  &    $-$13.58  &    $-$14.88  &    $-$15.17  &    $-$15.33  &       877  &        254  &       178  \\  %  52649-1192-183
74  &    $-$15.24  &    $-$14.74  &   $-$15.85  &   $-$14.51  &     $-$14.79  &    $-$16.14  &   $-$15.09  &    $-$14.02  &    $-$15.20  &    $-$15.64  &    $-$15.64  &       898  &        155  &       208  \\  %  52973-1300-127
75  &    $-$16.02  &    $-$15.35  &  $<-$16.31  &   $-$15.14  &     $-$15.48  &   $<-$15.83  &   $-$15.64  &    $-$14.73  &    $-$15.86  &    $-$16.21  &    $-$16.26  &       870  &        259  &   \nodata  \\  %  52312-0832-397
76  &    $-$14.69  &   $<-$15.34  &   $-$15.05  &   $-$14.91  &     $-$14.50  &    $-$15.71  &   $-$14.48  &    $-$14.31  &    $-$15.00  &    $-$15.28  &    $-$15.40  &      1159  &        179  &       199  \\  %  52620-0899-367
77  &    $-$15.03  &   $<-$15.54  &   $-$15.61  &   $-$15.50  &     $-$14.94  &    $-$15.98  &   $-$14.85  &    $-$14.64  &    $-$15.01  &    $-$15.29  &    $-$15.37  &      1383  &        278  &       229  \\  %  51908-0450-108
78  &    $-$15.52  &    $-$14.67  &   $-$15.46  &   $-$14.77  &     $-$15.28  &    $-$16.36  &   $-$14.88  &    $-$14.21  &    $-$15.33  &    $-$15.88  &    $-$16.04  &      1023  &        131  &       212  \\  %  52976-1301-471
79  &    $-$15.61  &    $-$14.81  &   $-$15.54  &   $-$14.89  &     $-$15.13  &   $<-$15.96  &  $<-$15.18  &    $-$14.40  &   $<-$15.72  &   $<-$16.01  &     \nodata  &       744  &        665  &   \nodata  \\  %  52652-1193-563
80  &    $-$15.52  &    $-$15.26  &  $<-$15.88  &   $-$15.17  &     $-$15.44  &   $<-$16.14  &   $-$15.29  &    $-$14.58  &    $-$15.35  &    $-$15.89  &    $-$15.88  &       535  &        341  &       251  \\  %  52707-0937-066
81  &    $-$15.26  &    $-$14.85  &   $-$15.42  &   $-$14.80  &     $-$15.18  &    $-$16.14  &   $-$14.79  &    $-$14.21  &    $-$15.08  &    $-$15.52  &    $-$15.63  &       824  &        211  &       174  \\  %  52707-0991-391
82  &    $-$15.20  &    $-$15.06  &   $-$15.28  &   $-$14.94  &     $-$14.98  &    $-$15.97  &   $-$14.62  &    $-$14.35  &    $-$14.95  &    $-$15.40  &    $-$15.56  &      1261  &        268  &       132  \\  %  52707-0991-268
83  &    $-$15.67  &   $<-$15.28  &   $-$15.50  &  $<-$15.55  &     $-$15.09  &   $<-$16.06  &   $-$14.83  &    $-$14.83  &    $-$15.05  &    $-$15.90  &    $-$15.85  &      1720  &        276  &       246  \\  %  52000-0474-225
84  &    $-$15.71  &   $<-$15.39  &   $-$15.91  &   $-$15.59  &     $-$15.55  &   $<-$16.11  &   $-$15.17  &    $-$15.08  &    $-$15.53  &    $-$15.88  &    $-$15.90  &      1715  &        163  &       257  \\  %  51929-0473-619
85  &    $-$15.67  &    $-$14.73  &   $-$15.89  &   $-$14.77  &     $-$15.01  &    $-$16.00  &   $-$15.36  &    $-$14.23  &    $-$15.68  &    $-$15.81  &    $-$16.05  &       519  &        397  &        93  \\  %  52707-0991-061
86  &    $-$15.38  &    $-$15.01  &  $<-$15.95  &   $-$15.14  &     $-$14.70  &    $-$15.69  &   $-$15.18  &    $-$14.19  &    $-$15.07  &    $-$15.54  &    $-$15.72  &      1135  &        650  &       305  \\  %  53050-1303-300
87  &    $-$15.18  &    $-$14.49  &   $-$15.43  &   $-$14.30  &     $-$14.46  &    $-$15.96  &   $-$14.87  &    $-$13.82  &    $-$15.08  &    $-$15.52  &    $-$15.60  &       840  &        195  &       209  \\  %  52266-0555-049
88  &    $-$15.74  &    $-$14.79  &   $-$15.85  &   $-$14.97  &     $-$15.16  &   $<-$16.22  &   $-$15.24  &    $-$14.41  &    $-$15.21  &    $-$15.90  &    $-$15.92  &      1169  &        296  &       197  \\  %  51915-0453-310
89  &    $-$15.83  &    $-$15.04  &   $-$15.61  &   $-$14.99  &     $-$15.45  &   $<-$16.06  &   $-$15.06  &    $-$14.51  &    $-$15.44  &    $-$15.92  &    $-$15.83  &       912  &        148  &        93  \\  %  52264-0569-634
90  &    $-$15.59  &   $<-$15.46  &  $<-$16.16  &   $-$15.60  &     $-$15.43  &   $<-$16.02  &   $-$15.62  &    $-$15.21  &    $-$15.64  &   $<-$16.41  &     \nodata  &       898  &        221  &   \nodata  \\  %  52725-1215-114
91  &    $-$14.87  &    $-$14.68  &   $-$15.14  &   $-$14.69  &     $-$14.39  &    $-$15.63  &   $-$14.47  &    $-$14.18  &    $-$14.72  &    $-$15.16  &    $-$15.27  &       805  &        181  &       184  \\  %  52724-1234-390
92  &    $-$15.59  &    $-$14.43  &   $-$15.52  &   $-$14.60  &     $-$14.88  &    $-$15.50  &   $-$14.64  &    $-$14.11  &    $-$15.25  &    $-$15.81  &    $-$16.00  &      1054  &        216  &       203  \\  %  51910-0486-059
93  &     \nodata  &    $-$14.64  &   $-$14.57  &   $-$13.88  &     $-$13.37  &    $-$14.61  &   $-$13.94  &    $-$13.33  &    $-$14.04  &    $-$14.50  &    $-$14.51  &      1807  &        315  &       328  \\  %  52757-1305-179
94  &    $-$15.18  &    $-$15.10  &  $<-$16.02  &   $-$15.48  &     $-$15.62  &    $-$15.73  &   $-$15.53  &    $-$15.10  &    $-$15.89  &    $-$15.64  &    $-$15.72  &      2040  &        132  &       346  \\  %  51943-0487-424
95  &    $-$15.31  &   $<-$15.35  &   $-$15.82  &   $-$15.20  &     $-$15.09  &   $<-$15.89  &   $-$15.14  &    $-$14.68  &    $-$15.42  &    $-$15.77  &    $-$15.81  &      1365  &        239  &       307  \\  %  52725-0994-490
96  &    $-$14.80  &   $<-$15.34  &   $-$15.20  &  $<-$15.71  &     $-$15.43  &    $-$15.96  &   $-$14.69  &    $-$14.88  &    $-$15.17  &    $-$15.31  &    $-$15.48  &      1580  &         88  &       121  \\  %  52998-1596-344
97  &    $-$15.05  &   $<-$15.32  &   $-$15.16  &  $<-$15.67  &     $-$14.16  &    $-$15.39  &   $-$14.60  &    $-$14.48  &    $-$14.80  &    $-$15.22  &    $-$15.33  &      1245  &        437  &       241  \\  %  52317-0558-282
98  &    $-$14.95  &    $-$14.64  &   $-$15.01  &   $-$14.29  &     $-$14.08  &    $-$15.44  &   $-$14.22  &    $-$13.68  &    $-$15.29  &    $-$15.58  &    $-$15.61  &      1049  &        139  &       151  \\  %  52709-1216-120
99  &   $<-$16.29  &    $-$14.90  &   $-$16.16  &   $-$15.16  &     $-$15.66  &   $<-$16.05  &  $<-$15.55  &    $-$14.69  &   $<-$15.95  &   $<-$15.83  &   $<-$15.57  &       663  &        163  &   \nodata  \\  %  52282-0769-062
100  &   $-$15.46  &    $-$15.25  &   $-$15.73  &   $-$15.16  &     $-$14.98  &    $-$15.91  &   $-$15.07  &    $-$14.55  &    $-$15.39  &    $-$15.72  &    $-$15.93  &      1097  &        197  &       200  \\  %  51633-0268-085
101  &   $-$15.43  &   $<-$15.39  &   $-$15.91  &   $-$15.15  &     $-$14.87  &    $-$16.25  &   $-$15.26  &    $-$14.56  &    $-$15.19  &    $-$15.81  &    $-$15.80  &       669  &        165  &       172  \\  %  52652-0945-172
102  &   $-$15.03  &    $-$15.18  &   $-$15.37  &   $-$14.82  &     $-$14.91  &    $-$15.71  &   $-$14.72  &    $-$14.21  &    $-$15.16  &    $-$15.40  &    $-$15.55  &       746  &        223  &       174  \\  %  52993-1426-132
103  &   $-$15.45  &    $-$15.25  &   $-$16.00  &   $-$15.00  &     $-$14.55  &    $-$15.79  &   $-$15.29  &    $-$14.43  &    $-$15.09  &    $-$15.72  &    $-$15.68  &       847  &        301  &       250  \\  %  52317-0558-611
104  &   $-$15.51  &    $-$15.27  &   $-$15.95  &   $-$14.83  &     $-$15.13  &   $<-$16.02  &   $-$15.78  &    $-$14.23  &   $<-$16.10  &     \nodata  &     \nodata  &       820  &        159  &   \nodata  \\  %  51909-0270-490
105  &   $-$15.01  &    $-$15.14  &   $-$15.56  &   $-$14.96  &     $-$14.49  &    $-$15.55  &   $-$14.86  &    $-$14.48  &    $-$15.21  &    $-$15.47  &    $-$15.44  &      1164  &        387  &       351  \\  %  51883-0271-277
106  &   $-$14.51  &    $-$15.11  &   $-$14.80  &   $-$14.53  &     $-$13.59  &    $-$15.10  &   $-$14.31  &    $-$13.83  &    $-$14.63  &    $-$15.01  &    $-$15.01  &       601  &        191  &       187  \\  %  53034-1357-543
107  &   $-$15.38  &   $<-$15.35  &   $-$15.92  &  $<-$15.65  &     $-$15.36  &   $<-$16.12  &   $-$15.20  &    $-$15.04  &    $-$15.51  &    $-$15.94  &    $-$16.17  &      1648  &        356  &       107  \\  %  51999-0503-098
108  &   $-$15.20  &    $-$15.50  &   $-$15.71  &   $-$15.69  &     $-$14.63  &    $-$16.00  &   $-$15.08  &    $-$15.07  &    $-$15.34  &    $-$15.63  &    $-$15.70  &      1477  &        107  &        95  \\  %  52998-1428-232
109  &   $-$14.99  &   $<-$15.43  &   $-$15.47  &   $-$15.20  &     $-$14.53  &    $-$15.69  &   $-$14.99  &    $-$14.46  &    $-$15.46  &    $-$15.49  &    $-$15.59  &      1614  &        172  &       176  \\  %  51999-0503-585
110  &  $<-$15.66  &   $<-$15.29  &  $<-$15.89  &   $-$15.40  &     $-$15.18  &    $-$15.69  &   $-$15.12  &    $-$14.93  &    $-$15.22  &    $-$15.70  &    $-$15.78  &       680  &        149  &       191  \\  %  52319-0575-199
111  &   $-$14.99  &   $<-$15.40  &   $-$15.53  &    \nodata  &     $-$15.67  &    $-$16.10  &   $-$15.02  &    $-$15.03  &    $-$15.46  &    $-$15.52  &    $-$15.83  &      1158  &        174  &       149  \\  %  52338-0874-499
112  &    \nodata  &   $<-$15.13  &   $-$15.23  &   $-$14.63  &     $-$14.37  &    $-$15.33  &   $-$14.49  &    $-$14.36  &    $-$14.63  &    $-$15.10  &    $-$15.15  &      2348  &        135  &       120  \\  %  51930-0489-193
113  &   $-$15.55  &    $-$15.06  &   $-$16.00  &   $-$14.87  &     $-$14.87  &    $-$16.40  &   $-$15.32  &    $-$14.31  &    $-$15.45  &    $-$15.81  &    $-$15.96  &      1002  &        216  &       169  \\  %  53089-1599-555
114  &   $-$14.99  &    $-$15.42  &   $-$15.29  &   $-$15.32  &     $-$15.04  &    $-$15.99  &   $-$14.70  &    $-$14.72  &    $-$15.09  &    $-$15.42  &    $-$15.51  &      1155  &        227  &       165  \\  %  52367-0577-414
115  &   $-$15.38  &   $<-$15.26  &  $<-$16.12  &   $-$15.31  &     $-$15.30  &   $<-$15.98  &   $-$15.27  &    $-$14.80  &    $-$15.37  &    $-$15.82  &    $-$16.05  &      1359  &        173  &       181  \\  %  52376-0773-258
116  &   $-$15.03  &   $<-$15.38  &   $-$15.39  &   $-$14.99  &     $-$14.83  &    $-$16.05  &   $-$14.80  &    $-$14.41  &    $-$15.21  &    $-$15.45  &    $-$15.61  &      1483  &        169  &       158  \\  %  52428-0948-259
117  &   $-$15.21  &    $-$14.61  &   $-$15.20  &   $-$14.71  &     $-$15.10  &    $-$15.90  &   $-$14.55  &    $-$14.09  &    $-$15.12  &    $-$15.46  &    $-$15.59  &       853  &        297  &       210  \\  %  51910-0275-312
118  &   $-$14.56  &    $-$14.55  &   $-$14.91  &   $-$14.33  &     $-$13.90  &    $-$15.22  &   $-$14.27  &    $-$13.80  &    $-$14.45  &    $-$14.85  &    $-$14.87  &      1224  &        255  &       257  \\  %  53115-1601-427
119  &   $-$15.19  &   $<-$15.32  &   $-$15.40  &    \nodata  &     $-$14.99  &    $-$16.16  &   $-$14.78  &    $-$15.01  &    $-$15.00  &    $-$15.42  &    $-$15.53  &      1635  &        187  &       170  \\  %  53047-1361-020
120  &   $-$15.39  &    $-$15.24  &   $-$16.16  &   $-$15.01  &     $-$14.76  &    $-$16.20  &   $-$15.54  &    $-$14.45  &    $-$15.35  &   $<-$15.95  &    $-$16.03  &       949  &        269  &   \nodata  \\  %  52669-0876-497
121  &   $-$15.46  &   $<-$15.38  &   $-$15.44  &   $-$15.57  &     $-$15.20  &    $-$15.73  &   $-$14.89  &    $-$14.88  &    $-$15.10  &    $-$15.63  &    $-$15.65  &       720  &        171  &       186  \\  %  53054-1436-303
122  &   $-$15.00  &    $-$15.24  &   $-$15.02  &   $-$15.15  &     $-$14.95  &    $-$15.78  &   $-$14.40  &    $-$14.54  &    $-$14.80  &    $-$15.18  &    $-$15.35  &      1101  &        265  &       127  \\  %  52643-0963-626
123  &   $-$15.34  &    $-$14.41  &   $-$15.50  &   $-$14.67  &     $-$15.26  &    $-$15.79  &   $-$14.74  &    $-$14.15  &    $-$15.15  &    $-$15.63  &    $-$15.57  &       621  &        437  &       137  \\  %  52646-1002-117
124  &   $-$15.37  &   $<-$15.31  &   $-$16.08  &   $-$15.38  &     $-$14.79  &    $-$15.99  &   $-$15.27  &    $-$14.65  &    $-$15.31  &    $-$15.80  &    $-$15.75  &      1442  &        210  &       194  \\  %  52723-1220-172
125  &   $-$14.09  &    $-$15.20  &   $-$14.60  &   $-$14.54  &     $-$13.99  &    $-$15.30  &   $-$14.08  &    $-$13.92  &    $-$14.46  &    $-$14.68  &    $-$14.83  &       600  &        325  &       330  \\  %  53054-1436-523
126  &   $-$15.16  &    $-$14.84  &   $-$15.80  &   $-$14.79  &     $-$14.80  &    $-$15.81  &   $-$15.18  &    $-$14.35  &    $-$15.13  &    $-$15.50  &    $-$15.54  &       932  &        399  &       308  \\  %  52751-1221-253
127  &   $-$15.26  &    $-$14.36  &   $-$15.22  &   $-$14.49  &     $-$14.90  &    $-$15.72  &   $-$14.61  &    $-$13.96  &    $-$14.86  &    $-$15.35  &    $-$15.36  &       759  &        461  &       151  \\  %  52356-0581-254
128  &   $-$15.27  &    $-$14.49  &   $-$15.37  &   $-$14.61  &     $-$14.88  &    $-$15.90  &   $-$14.63  &    $-$14.13  &    $-$14.88  &    $-$15.44  &    $-$15.59  &       845  &        259  &       180  \\  %  53078-1604-332
129  &   $-$16.12  &   $<-$15.51  &   $-$15.78  &   $-$15.18  &     $-$15.36  &   $<-$15.88  &   $-$15.14  &    $-$14.66  &    $-$15.50  &    $-$15.99  &    $-$16.02  &      1225  &        297  &       238  \\  %  51900-0278-279
130  &   $-$15.20  &   $<-$15.43  &   $-$15.27  &   $-$15.20  &     $-$15.07  &   $<-$16.03  &   $-$14.70  &    $-$14.54  &    $-$14.98  &    $-$15.42  &    $-$15.63  &      1044  &        401  &       258  \\  %  53078-1604-242
131  &   $-$14.74  &    $-$15.01  &   $-$14.92  &   $-$14.84  &     $-$14.52  &    $-$15.62  &   $-$14.30  &    $-$14.31  &    $-$14.62  &    $-$14.97  &    $-$15.12  &      1006  &        214  &       142  \\  %  52374-0509-143
132  &   $-$15.02  &    $-$14.75  &   $-$15.67  &   $-$14.59  &     $-$14.64  &    $-$15.76  &   $-$15.05  &    $-$14.01  &    $-$14.91  &    $-$15.45  &    $-$15.65  &       973  &        213  &       241  \\  %  52374-0509-508
133  &  $<-$15.64  &    $-$15.10  &   $-$16.08  &   $-$15.18  &     $-$15.10  &   $<-$16.07  &   $-$15.46  &    $-$14.72  &    $-$15.55  &    $-$15.82  &    $-$16.03  &      1713  &        311  &       376  \\  %  53046-1437-636
134  &   $-$15.19  &   $<-$15.31  &   $-$15.41  &   $-$15.45  &     $-$14.93  &    $-$16.13  &   $-$14.78  &    $-$14.83  &    $-$15.19  &    $-$15.58  &    $-$15.58  &      1547  &        171  &       170  \\  %  52646-0964-636
135  &   $-$15.33  &   $<-$15.34  &   $-$15.68  &   $-$15.68  &     $-$15.13  &   $<-$15.71  &   $-$15.04  &    $-$14.71  &    $-$15.21  &    $-$15.66  &    $-$15.73  &      1392  &        220  &       162  \\  %  52649-1012-401
136  &   $-$15.03  &    $-$15.19  &   $-$15.28  &   $-$14.92  &     $-$14.60  &    $-$16.23  &   $-$14.67  &    $-$14.35  &    $-$14.98  &    $-$15.47  &    $-$15.47  &       715  &        541  &       280  \\  %  52381-0510-198
137  &   $-$14.81  &    $-$14.63  &   $-$15.17  &   $-$14.50  &     $-$14.58  &    $-$15.73  &   $-$14.54  &    $-$14.04  &    $-$14.87  &    $-$15.21  &    $-$15.36  &      1180  &        158  &       139  \\  %  52649-1012-133
138  &   $-$15.80  &    $-$15.37  &  $<-$16.08  &   $-$15.41  &     $-$15.50  &    $-$16.43  &   $-$15.47  &    $-$14.99  &    $-$15.71  &    $-$16.36  &    $-$16.33  &       768  &         86  &   \nodata  \\  %  53084-1440-250
139  &   $-$15.88  &   $<-$15.43  &   $-$15.57  &   $-$15.62  &     $-$15.57  &   $<-$16.02  &   $-$15.00  &    $-$15.18  &    $-$15.41  &    $-$15.78  &    $-$15.90  &      1333  &        213  &       118  \\  %  52707-1013-169
140  &   $-$14.70  &    $-$15.04  &   $-$15.24  &   $-$14.92  &     $-$15.02  &    $-$15.15  &   $-$14.65  &    $-$14.25  &    $-$15.44  &    $-$15.09  &    $-$15.19  &      1395  &        519  &       345  \\  %  53084-1440-512
141  &   $-$14.52  &   $<-$15.13  &   $-$15.37  &  $<-$15.42  &     $-$14.28  &    $-$15.08  &   $-$14.73  &    $-$14.27  &    $-$14.39  &    $-$14.68  &    $-$14.75  &      1774  &        599  &       412  \\  %  52365-0879-328
142  &   $-$14.94  &    $-$14.65  &   $-$15.32  &   $-$14.50  &     $-$14.35  &    $-$15.63  &   $-$14.74  &    $-$13.93  &    $-$14.93  &    $-$15.29  &    $-$15.39  &       913  &        261  &       209  \\  %  53062-1365-124
143  &   $-$14.89  &    $-$14.89  &   $-$15.43  &   $-$14.59  &     $-$14.37  &    $-$15.59  &   $-$14.72  &    $-$13.96  &    $-$14.86  &    $-$15.31  &    $-$15.28  &      1266  &        238  &       238  \\  %  52636-0511-031
144  &   $-$15.50  &   $<-$15.40  &   $-$15.76  &   $-$15.47  &     $-$15.06  &    $-$15.87  &   $-$15.14  &    $-$14.71  &    $-$15.28  &    $-$15.66  &    $-$15.97  &      1049  &        183  &       193  \\  %  52781-1223-409
145  &   $-$14.85  &   $<-$15.24  &   $-$15.20  &   $-$15.11  &     $-$14.34  &    $-$15.59  &   $-$14.69  &    $-$14.13  &    $-$14.67  &    $-$15.11  &    $-$15.16  &      1857  &        482  &       234  \\  %  53083-1441-619
146  &   $-$15.01  &   $<-$15.18  &   $-$15.29  &   $-$14.78  &     $-$14.40  &    $-$15.71  &   $-$14.72  &    $-$14.22  &    $-$14.70  &    $-$15.18  &    $-$15.20  &      1473  &        256  &       258  \\  %  52365-0879-200
147  &   $-$15.16  &   $<-$15.45  &   $-$15.66  &   $-$15.60  &     $-$15.28  &    $-$15.68  &   $-$14.84  &    $-$14.67  &    $-$15.06  &    $-$15.24  &    $-$15.31  &       772  &        502  &       331  \\  %  53050-1442-263
148  &   $-$15.07  &   $<-$15.41  &   $-$15.44  &   $-$15.35  &     $-$14.39  &    $-$15.77  &   $-$14.87  &    $-$14.71  &    $-$14.83  &    $-$15.40  &    $-$15.44  &       726  &        174  &       180  \\  %  52409-0952-228
149  &   $-$15.08  &    $-$15.17  &   $-$15.30  &   $-$14.90  &     $-$14.55  &    $-$15.95  &   $-$14.65  &    $-$14.45  &    $-$14.84  &    $-$15.34  &    $-$15.37  &      1208  &        166  &       207  \\  %  52059-0597-560
150  &   $-$15.39  &    $-$14.53  &   $-$15.69  &   $-$14.51  &     $-$14.77  &   $<-$16.12  &   $-$14.87  &    $-$14.02  &    $-$15.02  &    $-$15.58  &    $-$15.64  &       969  &        161  &       253  \\  %  53055-1443-608
151  &   $-$15.04  &    $-$14.47  &   $-$15.67  &   $-$14.39  &     $-$14.64  &    $-$15.94  &   $-$14.85  &    $-$13.98  &    $-$15.05  &    $-$15.43  &    $-$15.55  &      1255  &        253  &       206  \\  %  53055-1443-009
152  &   $-$15.74  &   $<-$15.49  &   $-$15.91  &   $-$15.72  &     $-$15.64  &   $<-$15.82  &   $-$15.09  &    $-$15.16  &    $-$15.42  &    $-$16.00  &    $-$16.00  &      1628  &        186  &       255  \\  %  53083-1607-513
153  &   $-$15.17  &    $-$14.30  &   $-$15.63  &   $-$14.39  &     $-$14.91  &    $-$15.76  &   $-$14.87  &    $-$13.92  &    $-$14.92  &    $-$15.48  &    $-$15.53  &       601  &        214  &       156  \\  %  51994-0514-331
154  &   $-$15.01  &   $<-$15.37  &   $-$15.04  &   $-$14.80  &     $-$14.75  &    $-$15.84  &   $-$14.33  &    $-$14.34  &    $-$14.60  &    $-$15.06  &    $-$15.20  &      1916  &        195  &       284  \\  %  52282-0328-197
155  &  $<-$16.20  &    $-$14.65  &  $<-$16.30  &   $-$15.08  &     $-$15.73  &   $<-$15.81  &  $<-$15.78  &    $-$14.56  &   $<-$15.88  &   $<-$16.10  &   $<-$16.08  &       634  &    \nodata  &   \nodata  \\  %  53083-1367-481
156  &   $-$15.01  &    $-$14.16  &  $<-$15.68  &   $-$14.14  &     $-$14.80  &    $-$15.94  &   $-$14.55  &    $-$13.61  &    $-$15.12  &    $-$15.56  &    $-$15.69  &       815  &        319  &       217  \\  %  52316-0598-301
157  &   $-$14.76  &    $-$15.21  &   $-$15.14  &   $-$14.85  &     $-$14.91  &    $-$15.99  &   $-$14.57  &    $-$14.39  &    $-$15.03  &    $-$15.20  &    $-$15.37  &      1153  &        195  &       218  \\  %  52282-0328-107
158  &   $-$14.34  &   $<-$15.27  &   $-$14.75  &   $-$15.09  &     $-$14.63  &    $-$15.86  &   $-$14.13  &    $-$14.10  &    $-$14.96  &    $-$15.00  &    $-$15.17  &       999  &         97  &       114  \\  %  52734-1015-596
159  &   $-$15.05  &    $-$14.67  &   $-$15.23  &   $-$14.81  &     $-$14.94  &   $<-$15.84  &   $-$14.62  &    $-$14.26  &    $-$14.92  &    $-$15.39  &    $-$15.48  &       951  &        443  &       234  \\  %  53084-1368-285
160  &   $-$15.57  &    $-$14.88  &   $-$15.77  &   $-$14.92  &     $-$15.50  &   $<-$16.13  &   $-$15.10  &    $-$14.27  &    $-$15.24  &    $-$15.68  &    $-$15.79  &       622  &        280  &       165  \\  %  52734-1226-485
161  &   $-$15.22  &   $<-$15.34  &   $-$15.15  &   $-$15.27  &     $-$14.96  &    $-$15.97  &   $-$14.50  &    $-$14.63  &    $-$14.90  &    $-$15.38  &    $-$15.51  &      1224  &        228  &       175  \\  %  52056-0329-169
162  &   $-$15.46  &   $<-$15.35  &   $-$15.55  &   $-$15.05  &     $-$14.96  &    $-$16.08  &   $-$15.11  &    $-$14.48  &    $-$15.46  &    $-$15.68  &    $-$15.74  &      1334  &        197  &       203  \\  %  52367-0880-032
163  &   $-$14.63  &    $-$14.67  &   $-$14.96  &   $-$14.58  &     $-$14.18  &    $-$15.40  &   $-$14.38  &    $-$13.96  &    $-$14.58  &    $-$15.02  &    $-$15.06  &      1122  &        188  &       182  \\  %  52781-1312-121
164  &   $-$14.34  &    $-$13.54  &   $-$14.23  &   $-$13.46  &     $-$13.96  &    $-$15.08  &   $-$13.58  &    $-$12.96  &    $-$13.96  &    $-$14.51  &    $-$14.59  &       984  &        207  &       192  \\  %  53080-1446-129
165  &   $-$15.47  &    $-$14.63  &   $-$15.78  &   $-$14.67  &     $-$15.04  &    $-$15.89  &   $-$14.99  &    $-$14.17  &    $-$15.24  &    $-$15.68  &    $-$15.83  &       787  &        273  &       196  \\  %  52411-0953-077
166  &   $-$15.06  &   $<-$15.36  &   $-$15.33  &   $-$15.22  &     $-$15.03  &    $-$16.02  &   $-$14.66  &    $-$14.60  &    $-$14.98  &    $-$15.38  &    $-$15.53  &      1420  &        149  &       212  \\  %  52442-0969-445
167  &   $-$15.07  &   $<-$15.31  &   $-$15.26  &   $-$15.41  &     $-$14.79  &    $-$16.06  &   $-$14.64  &    $-$14.78  &    $-$14.85  &    $-$15.37  &    $-$15.45  &      1469  &        174  &       138  \\  %  52367-0332-604
168  &   $-$15.25  &   $<-$15.43  &   $-$15.58  &  $<-$15.67  &     $-$14.82  &    $-$15.58  &   $-$14.91  &    $-$14.99  &    $-$15.08  &    $-$15.42  &    $-$15.47  &      2046  &        259  &       296  \\  %  53090-1370-483
169  &   $-$14.69  &    $-$15.03  &   $-$15.00  &   $-$14.69  &     $-$14.31  &    $-$15.52  &   $-$14.36  &    $-$14.18  &    $-$14.57  &    $-$15.00  &    $-$15.14  &       917  &        150  &       192  \\  %  52282-0518-218
170  &   $-$14.81  &   $<-$15.24  &   $-$15.03  &   $-$15.47  &     $-$14.17  &    $-$15.32  &   $-$14.45  &    $-$14.65  &    $-$14.70  &    $-$15.11  &    $-$15.22  &      1513  &        268  &       184  \\  %  52409-0955-466
171  &   $-$15.53  &    $-$14.86  &   $-$15.64  &   $-$15.19  &     $-$15.46  &   $<-$16.20  &   $-$14.91  &    $-$14.69  &    $-$15.24  &    $-$15.83  &    $-$15.81  &      1074  &        346  &       320  \\  %  52413-0970-558
172  &   $-$15.23  &   $<-$15.29  &   $-$15.42  &  $<-$15.66  &     $-$14.94  &    $-$16.04  &   $-$14.79  &    $-$14.70  &    $-$15.00  &    $-$15.55  &    $-$15.65  &      1752  &        183  &       170  \\  %  52430-0883-606
173  &   $-$14.86  &    $-$14.88  &   $-$15.20  &   $-$14.66  &     $-$14.76  &    $-$15.65  &   $-$14.43  &    $-$14.09  &    $-$14.73  &    $-$15.12  &    $-$15.23  &      1233  &        290  &       240  \\  %  52672-1230-131
174  &    \nodata  &   $<-$15.12  &   $-$14.82  &   $-$14.29  &     $-$13.74  &    $-$15.11  &   $-$14.04  &    $-$13.58  &    $-$14.88  &    $-$15.15  &    $-$15.14  &       949  &        123  &       111  \\  %  52791-1315-568
175  &  $<-$15.47  &    $-$14.57  &   $-$15.66  &   $-$14.78  &     $-$15.23  &    $-$15.52  &   $-$15.06  &    $-$14.18  &    $-$15.45  &    $-$15.94  &    $-$16.18  &       655  &        249  &       104  \\  %  53140-1625-071
176  &   $-$15.72  &   $<-$15.51  &   $-$15.81  &   $-$15.59  &     $-$15.27  &   $<-$16.10  &   $-$15.25  &    $-$15.03  &    $-$15.51  &    $-$15.95  &    $-$15.98  &      1308  &        237  &       304  \\  %  53112-1452-157
177  &   $-$14.87  &   $<-$15.36  &   $-$15.30  &   $-$15.23  &     $-$14.69  &    $-$15.78  &   $-$14.69  &    $-$14.65  &    $-$15.18  &    $-$15.33  &    $-$15.49  &       812  &        176  &       156  \\  %  52342-0779-621
178  &   $-$15.51  &   $<-$15.44  &   $-$16.00  &  $<-$15.73  &     $-$15.25  &    $-$16.00  &   $-$15.38  &    $-$14.93  &    $-$15.35  &    $-$15.84  &    $-$16.07  &      1616  &        542  &       286  \\  %  52317-0600-437
179  &   $-$15.37  &   $<-$15.39  &   $-$15.58  &   $-$15.67  &     $-$15.15  &   $<-$16.07  &   $-$14.96  &    $-$14.71  &    $-$15.17  &    $-$15.84  &    $-$15.83  &       544  &        310  &       279  \\  %  51990-0289-625
180  &   $-$15.65  &    $-$14.64  &   $-$15.76  &   $-$14.81  &     $-$15.10  &    $-$16.35  &   $-$15.14  &    $-$14.25  &    $-$15.50  &    $-$16.06  &    $-$16.06  &       846  &        293  &       146  \\  %  52317-0600-043
181  &   $-$14.30  &    $-$14.58  &   $-$14.79  &   $-$14.33  &     $-$13.80  &    $-$15.14  &   $-$14.15  &    $-$13.72  &    $-$14.67  &    $-$14.93  &    $-$14.93  &       819  &        211  &       159  \\  %  51941-0290-021
182  &   $-$15.16  &   $<-$15.45  &   $-$15.30  &   $-$15.42  &     $-$15.03  &    $-$15.96  &   $-$14.71  &    $-$14.90  &    $-$14.99  &    $-$15.47  &    $-$15.59  &      1773  &        218  &       169  \\  %  51928-0291-375
183  &   $-$15.29  &    $-$15.25  &   $-$15.20  &   $-$15.22  &     $-$15.14  &   $<-$16.10  &   $-$14.58  &    $-$14.77  &    $-$14.99  &    $-$15.41  &    $-$15.56  &      1434  &        173  &       141  \\  %  52765-1317-421
184  &   $-$15.55  &    $-$14.59  &   $-$15.65  &   $-$14.75  &     $-$15.40  &   $<-$16.13  &   $-$15.05  &    $-$14.25  &    $-$15.52  &    $-$15.89  &    $-$15.88  &       813  &        239  &       179  \\  %  52379-0885-107
185  &   $-$14.41  &   $<-$15.35  &   $-$14.91  &   $-$14.92  &     $-$14.02  &    $-$15.45  &   $-$14.34  &    $-$14.19  &    $-$15.02  &    $-$15.12  &    $-$15.25  &       713  &        170  &       169  \\  %  52373-0781-076
186  &   $-$14.27  &   $<-$15.27  &   $-$14.71  &   $-$14.76  &     $-$14.07  &    $-$15.41  &   $-$14.18  &    $-$14.12  &    $-$14.77  &    $-$14.88  &    $-$15.00  &      1120  &        146  &       172  \\  %  51997-0337-425
187  &   $-$14.73  &   $<-$15.32  &   $-$15.00  &   $-$15.32  &     $-$14.29  &    $-$15.39  &   $-$14.35  &    $-$14.18  &    $-$14.61  &    $-$15.22  &    $-$15.23  &       632  &        232  &       245  \\  %  52316-0601-533
188  &   $-$15.42  &    $-$15.25  &   $-$15.84  &   $-$15.56  &     $-$14.96  &    $-$15.94  &   $-$15.09  &    $-$14.69  &    $-$15.18  &    $-$15.65  &    $-$15.73  &      1521  &        300  &       246  \\  %  53116-1457-236
189  &   $-$15.15  &   $<-$15.41  &   $-$15.67  &   $-$15.03  &     $-$14.80  &    $-$15.95  &   $-$15.03  &    $-$14.56  &    $-$15.28  &    $-$15.66  &    $-$15.74  &      1048  &        385  &       262  \\  %  52736-1279-075
190  &   $-$15.27  &   $<-$15.30  &   $-$15.42  &   $-$15.50  &     $-$15.21  &   $<-$16.13  &   $-$14.81  &    $-$14.65  &    $-$15.18  &    $-$15.57  &    $-$15.66  &      1757  &        241  &       232  \\  %  51994-0293-525
191  &   $-$14.74  &    $-$15.37  &   $-$14.98  &   $-$15.18  &     $-$14.87  &    $-$15.77  &   $-$14.40  &    $-$14.59  &    $-$14.84  &    $-$15.18  &    $-$15.27  &       665  &        266  &       266  \\  %  51986-0294-296
192  &   $-$15.26  &    $-$15.31  &   $-$15.67  &   $-$15.05  &     $-$14.91  &    $-$15.90  &   $-$15.00  &    $-$14.45  &    $-$15.09  &    $-$15.62  &    $-$15.68  &      1434  &        317  &       156  \\  %  53083-1374-542
193  &   $-$14.75  &    $-$15.12  &   $-$15.23  &   $-$14.73  &     $-$14.18  &    $-$15.38  &   $-$14.56  &    $-$13.89  &    $-$14.58  &    $-$15.02  &    $-$15.10  &      1199  &        238  &       222  \\  %  52376-0887-100
194  &   $-$15.58  &    $-$14.68  &   $-$15.99  &   $-$14.87  &     $-$15.37  &     \nodata  &   $-$15.73  &    $-$14.42  &    $-$15.87  &    $-$15.94  &    $-$16.16  &       675  &        587  &        70  \\  %  52027-0524-640
195  &   $-$15.62  &    $-$15.05  &   $-$15.55  &   $-$15.39  &     $-$15.54  &   $<-$16.18  &   $-$14.95  &    $-$15.01  &    $-$15.34  &    $-$15.86  &    $-$16.13  &       863  &        205  &       172  \\  %  52072-0602-051
196  &   $-$15.13  &    $-$14.80  &   $-$15.30  &   $-$14.28  &     $-$14.36  &    $-$15.73  &   $-$14.73  &    $-$13.64  &    $-$14.80  &    $-$15.21  &    $-$15.26  &      1585  &        124  &       167  \\  %  52295-0525-091
197  &   $-$14.62  &   $<-$15.24  &   $-$15.19  &   $-$14.94  &     $-$14.34  &    $-$15.48  &   $-$14.61  &    $-$14.31  &    $-$14.74  &    $-$15.09  &    $-$15.15  &       672  &        204  &       197  \\  %  52338-0850-585
198  &   $-$15.12  &    $-$14.50  &   $-$15.13  &   $-$14.62  &     $-$14.79  &   $<-$15.81  &   $-$14.50  &    $-$14.01  &    $-$14.57  &    $-$15.19  &    $-$15.29  &       779  &        539  &       359  \\  %  53142-1697-464
199  &   $-$15.34  &    $-$14.73  &   $-$15.26  &   $-$14.91  &     $-$14.78  &    $-$15.99  &   $-$14.66  &    $-$14.31  &    $-$15.26  &    $-$15.60  &    $-$15.72  &       867  &        243  &       135  \\  %  53112-1773-411
200  &   $-$14.57  &    $-$15.08  &   $-$15.04  &   $-$14.63  &     $-$13.87  &    $-$15.29  &   $-$14.44  &    $-$14.03  &    $-$15.05  &    $-$15.15  &    $-$15.15  &       895  &        202  &       275  \\  %  53112-1773-226
201  &   $-$14.91  &   $<-$15.31  &   $-$15.10  &   $-$14.85  &     $-$14.78  &    $-$15.73  &   $-$14.42  &    $-$14.17  &    $-$14.65  &    $-$15.12  &    $-$15.18  &      1314  &        343  &       240  \\  %  52312-0526-309
202  &   $-$15.20  &    $-$15.08  &   $-$15.82  &   $-$14.88  &     $-$14.72  &    $-$15.81  &   $-$15.22  &    $-$14.36  &    $-$15.05  &    $-$15.60  &    $-$15.51  &       993  &        280  &       287  \\  %  52759-1282-271
203  &   $-$15.23  &    $-$14.29  &   $-$15.16  &   $-$14.34  &     $-$14.90  &   $<-$15.89  &   $-$14.59  &    $-$14.00  &    $-$14.86  &    $-$15.51  &    $-$15.57  &      1293  &        170  &       147  \\  %  53138-1460-004
204  &   $-$14.22  &    $-$14.55  &   $-$14.51  &   $-$14.51  &     $-$14.15  &    $-$15.38  &   $-$13.90  &    $-$13.86  &    $-$14.29  &    $-$14.65  &    $-$14.76  &       842  &        254  &       157  \\  %  53146-1698-257
205  &   $-$14.63  &   $<-$15.29  &   $-$14.91  &   $-$14.94  &     $-$14.39  &    $-$15.42  &   $-$14.28  &    $-$14.14  &    $-$14.51  &    $-$15.02  &    $-$15.04  &       627  &        230  &       173  \\  %  53089-1376-087
206  &    \nodata  &   $<-$15.11  &   $-$15.03  &   $-$15.01  &     $-$14.44  &    $-$15.36  &   $-$14.41  &    $-$14.27  &    $-$14.69  &    $-$14.81  &    $-$14.91  &      1388  &        266  &       272  \\  %  52375-0852-394
207  &   $-$14.42  &    $-$15.24  &   $-$14.92  &   $-$15.02  &     $-$14.27  &    $-$15.57  &   $-$14.41  &    $-$14.48  &    $-$15.21  &    $-$15.17  &    $-$15.30  &       915  &        351  &       163  \\  %  51988-0496-091
208  &   $-$14.82  &    $-$15.10  &   $-$15.20  &   $-$15.05  &     $-$13.91  &    $-$15.16  &   $-$14.77  &    $-$14.25  &    $-$15.04  &    $-$15.18  &    $-$15.24  &       967  &        266  &       245  \\  %  52426-0911-283
209  &   $-$15.20  &    $-$15.15  &   $-$15.31  &   $-$15.27  &     $-$15.24  &    $-$15.97  &   $-$14.69  &    $-$14.67  &    $-$15.10  &    $-$15.43  &    $-$15.50  &       640  &        176  &       121  \\  %  52377-0910-144
210  &   $-$15.21  &   $<-$15.52  &   $-$15.39  &   $-$15.56  &     $-$15.11  &    $-$15.91  &   $-$14.65  &    $-$14.48  &    $-$14.96  &    $-$15.40  &    $-$15.51  &      1323  &        589  &       317  \\  %  52022-0528-152
211  &   $-$15.10  &   $<-$15.39  &   $-$15.49  &   $-$15.17  &     $-$14.74  &    $-$16.08  &   $-$14.88  &    $-$14.67  &    $-$15.89  &    $-$15.84  &    $-$16.01  &       519  &         98  &       106  \\  %  52764-1321-044
212  &   $-$15.40  &    $-$14.64  &   $-$15.79  &   $-$14.70  &     $-$14.98  &    $-$16.32  &   $-$15.05  &    $-$14.17  &    $-$15.13  &    $-$15.63  &    $-$15.76  &       776  &        273  &       130  \\  %  53091-1464-029
213  &   $-$15.09  &    $-$14.97  &   $-$15.30  &   $-$15.08  &     $-$14.67  &    $-$16.05  &   $-$14.73  &    $-$14.48  &    $-$14.99  &    $-$15.50  &    $-$15.54  &       635  &        277  &       170  \\  %  51671-0299-134
214  &   $-$14.91  &    $-$14.49  &   $-$15.33  &   $-$14.41  &     $-$14.67  &    $-$16.17  &   $-$14.62  &    $-$13.93  &    $-$14.79  &    $-$15.25  &    $-$15.30  &       928  &        188  &       217  \\  %  52762-1283-635
215  &   $-$15.00  &   $<-$15.45  &   $-$15.37  &   $-$15.31  &     $-$15.02  &    $-$16.13  &   $-$14.73  &    $-$14.82  &    $-$15.05  &    $-$15.43  &    $-$15.48  &      1195  &        350  &       136  \\  %  51943-0300-281
216  &    \nodata  &   $<-$14.84  &   $-$14.56  &    \nodata  &     $-$13.37  &    $-$14.45  &   $-$13.97  &    $-$13.85  &    $-$13.81  &    $-$14.35  &    $-$14.37  &      1847  &        424  &       323  \\  %  52079-0604-536
217  &   $-$14.62  &    $-$14.55  &   $-$15.05  &   $-$14.52  &     $-$14.18  &    $-$15.46  &   $-$14.46  &    $-$13.94  &    $-$14.59  &    $-$14.97  &    $-$15.00  &       621  &        252  &       207  \\  %  52736-1284-151
218  &   $-$14.78  &   $<-$15.31  &   $-$15.02  &   $-$15.25  &     $-$14.89  &    $-$15.86  &   $-$14.38  &    $-$14.66  &    $-$14.77  &    $-$15.18  &    $-$15.34  &      1111  &        150  &       126  \\  %  52026-0530-183
219  &   $-$14.98  &    $-$14.90  &   $-$15.02  &   $-$14.80  &     $-$14.72  &    $-$15.48  &   $-$14.36  &    $-$14.27  &    $-$14.70  &    $-$15.16  &    $-$15.23  &      1363  &        221  &       268  \\  %  52026-0530-541
220  &   $-$15.35  &    $-$15.10  &   $-$15.64  &   $-$15.10  &     $-$14.91  &    $-$15.84  &   $-$14.99  &    $-$14.54  &    $-$15.09  &    $-$15.59  &    $-$15.66  &       717  &        294  &       193  \\  %  51984-0498-344
221  &   $-$15.01  &    $-$14.60  &   $-$15.18  &   $-$14.46  &     $-$14.37  &    $-$15.76  &   $-$14.61  &    $-$13.92  &    $-$14.98  &    $-$15.77  &    $-$15.63  &       923  &        176  &       136  \\  %  51989-0497-014
222  &    \nodata  &   $<-$15.00  &   $-$13.86  &   $-$14.50  &     $-$13.12  &    $-$14.38  &   $-$13.27  &    $-$13.78  &    $-$13.64  &    $-$14.12  &    $-$14.16  &      1800  &        187  &       157  \\  %  52443-0915-437 ;UM625
223  &   $-$15.23  &    $-$15.19  &   $-$15.66  &   $-$15.17  &     $-$14.91  &    $-$16.31  &   $-$14.92  &    $-$14.39  &    $-$15.86  &    $-$15.85  &    $-$15.95  &      1251  &        182  &       255  \\  %  51688-0302-227
224  &  $<-$16.34  &    $-$15.02  &   $-$16.03  &   $-$15.10  &     $-$16.07  &     \nodata  &   $-$15.49  &    $-$14.62  &    $-$15.88  &   $<-$16.34  &   $<-$16.30  &      1179  &    \nodata  &   \nodata  \\  %  53178-1704-481
225  &   $-$15.75  &    $-$14.67  &   $-$16.14  &   $-$14.74  &     $-$15.00  &   $<-$16.10  &   $-$15.36  &    $-$14.18  &    $-$15.41  &    $-$15.86  &    $-$16.03  &       731  &        227  &       134  \\  %  51615-0303-302
226  &   $-$14.91  &   $<-$15.36  &   $-$15.13  &   $-$15.61  &     $-$15.13  &    $-$15.83  &   $-$14.49  &    $-$14.82  &    $-$14.83  &    $-$15.23  &    $-$15.35  &      1005  &        213  &       209  \\  %  53108-1394-391
227  &   $-$15.34  &    $-$14.97  &   $-$15.34  &   $-$15.45  &     $-$15.31  &    $-$16.03  &   $-$14.70  &    $-$14.96  &    $-$15.07  &    $-$15.63  &    $-$15.83  &       970  &        144  &       162  \\  %  51615-0303-435
228  &   $-$15.38  &   $<-$15.38  &   $-$16.09  &  $<-$15.81  &     $-$15.36  &   $<-$15.98  &   $-$15.26  &    $-$14.73  &    $-$15.35  &    $-$15.66  &    $-$15.91  &      1275  &        236  &       272  \\  %  52055-0583-174
229  &   $-$15.60  &    $-$15.16  &   $-$15.93  &   $-$15.01  &     $-$15.07  &   $<-$15.94  &   $-$15.18  &    $-$14.46  &    $-$15.30  &    $-$15.91  &    $-$15.85  &       743  &        279  &       138  \\  %  52728-1287-365
230  &   $-$14.89  &    $-$15.22  &   $-$15.39  &   $-$14.86  &     $-$14.53  &    $-$15.74  &   $-$14.76  &    $-$14.31  &    $-$15.14  &    $-$15.34  &    $-$15.55  &       823  &        150  &       157  \\  %  51988-0499-293
231  &   $-$15.00  &   $<-$15.43  &   $-$15.44  &    \nodata  &     $-$15.49  &    $-$16.06  &   $-$14.75  &    $-$14.84  &    $-$14.98  &    $-$15.39  &    $-$15.51  &      1235  &        270  &       260  \\  %  52365-0606-565
232  &   $-$14.75  &    $-$14.77  &   $-$15.24  &   $-$14.55  &     $-$14.69  &    $-$15.87  &   $-$14.64  &    $-$14.09  &    $-$15.08  &    $-$15.37  &    $-$15.50  &      1051  &        155  &       133  \\  %  51997-0534-047
233  &   $-$15.64  &    $-$15.17  &  $<-$16.00  &   $-$14.98  &     $-$15.33  &   $<-$16.11  &   $-$15.46  &    $-$14.42  &    $-$15.48  &    $-$15.98  &    $-$16.07  &       983  &        321  &       236  \\  %  53144-1644-094
234  &   $-$15.45  &   $<-$15.32  &   $-$16.08  &   $-$15.18  &     $-$15.07  &    $-$15.98  &   $-$15.46  &    $-$14.74  &    $-$15.21  &    $-$15.77  &    $-$15.82  &      1269  &        191  &       276  \\  %  53144-1644-048
235  &   $-$15.56  &    $-$15.11  &   $-$15.61  &   $-$15.18  &     $-$15.00  &   $<-$16.14  &   $-$15.05  &    $-$14.52  &    $-$15.40  &    $-$16.00  &    $-$16.10  &      1180  &        173  &       159  \\  %  52441-0790-230
236  &   $-$15.26  &   $<-$15.33  &   $-$15.76  &   $-$15.39  &     $-$14.93  &   $<-$16.07  &   $-$15.14  &    $-$14.69  &    $-$15.24  &    $-$15.78  &    $-$15.71  &      1527  &        237  &       240  \\  %  52441-0790-253
237  &   $-$15.86  &    $-$14.41  &   $-$15.64  &   $-$14.56  &     $-$14.89  &    $-$15.73  &   $-$14.96  &    $-$14.01  &    $-$15.23  &    $-$15.68  &    $-$15.83  &       860  &        280  &       141  \\  %  52731-1288-430
238  &   $-$15.19  &   $<-$15.30  &   $-$15.76  &   $-$15.45  &     $-$14.68  &    $-$15.74  &   $-$15.20  &    $-$14.39  &    $-$15.07  &    $-$15.30  &    $-$15.35  &      1428  &        230  &       305  \\  %  52781-1327-377
239  &   $-$15.23  &   $<-$15.33  &   $-$15.28  &   $-$14.88  &     $-$14.67  &    $-$15.83  &   $-$14.67  &    $-$14.33  &    $-$14.90  &    $-$15.38  &    $-$15.41  &      1227  &        232  &       169  \\  %  52023-0586-234
240  &   $-$15.11  &   $<-$15.43  &   $-$15.19  &   $-$15.25  &     $-$15.13  &    $-$16.23  &   $-$14.54  &    $-$14.75  &    $-$14.92  &    $-$15.35  &    $-$15.46  &       742  &        197  &       119  \\  %  52409-0919-223
241  &   $-$15.99  &    $-$15.12  &  $<-$16.28  &   $-$15.10  &     $-$15.40  &   $<-$16.19  &   $-$15.96  &    $-$14.60  &    $-$15.94  &    $-$16.21  &    $-$16.36  &       628  &        367  &   \nodata  \\  %  52441-0790-156
242  &   $-$15.36  &   $<-$15.37  &   $-$15.53  &   $-$15.21  &     $-$15.00  &    $-$15.95  &   $-$14.82  &    $-$14.58  &    $-$15.45  &    $-$15.66  &    $-$15.69  &      1137  &        297  &       217  \\  %  53172-1645-139
243  &   $-$15.39  &   $<-$15.33  &   $-$15.81  &  $<-$15.57  &     $-$15.35  &    $-$15.97  &   $-$15.14  &    $-$14.99  &    $-$15.28  &    $-$15.75  &    $-$15.85  &      2134  &        257  &       161  \\  %  52409-0919-512
244  &   $-$14.82  &    $-$14.61  &   $-$14.97  &   $-$14.64  &     $-$14.49  &    $-$15.63  &   $-$14.38  &    $-$13.98  &    $-$14.65  &    $-$15.02  &    $-$15.17  &       923  &        250  &       294  \\  %  52668-1162-156
245  &   $-$14.65  &    $-$14.38  &   $-$14.67  &   $-$14.27  &     $-$14.45  &    $-$15.57  &   $-$14.04  &    $-$13.84  &    $-$14.44  &    $-$14.88  &    $-$14.99  &      1171  &        191  &       173  \\  %  52411-0920-289
246  &   $-$14.61  &   $<-$15.28  &   $-$14.91  &   $-$15.18  &     $-$14.38  &    $-$15.52  &   $-$14.28  &    $-$14.41  &    $-$14.66  &    $-$14.95  &    $-$15.09  &       827  &        310  &       233  \\  %  53172-1645-626
247  &  $<-$16.06  &   $<-$15.34  &   $-$16.52  &   $-$15.40  &     $-$15.96  &   $<-$16.01  &   $-$15.89  &    $-$14.53  &   $<-$16.11  &   $<-$16.33  &   $<-$16.32  &      1593  &    \nodata  &   \nodata  \\  %  52081-0608-405
248  &   $-$15.67  &    $-$15.40  &   $-$16.05  &   $-$15.15  &     $-$15.12  &    $-$16.28  &   $-$15.08  &    $-$14.48  &    $-$16.24  &    $-$16.26  &    $-$16.20  &      1400  &        134  &   \nodata  \\  %  51662-0308-492
249  &   $-$15.09  &    $-$14.44  &   $-$15.38  &   $-$14.57  &     $-$14.61  &    $-$15.84  &   $-$14.85  &    $-$13.89  &    $-$15.05  &    $-$15.41  &    $-$15.53  &      1002  &        154  &       179  \\  %  52435-0791-511
250  &  $<-$15.69  &    $-$14.93  &   $-$15.95  &   $-$14.99  &     $-$15.63  &     \nodata  &   $-$15.30  &    $-$14.69  &   $<-$15.97  &   $<-$16.18  &     \nodata  &       934  &        467  &   \nodata  \\  %  51994-0309-071
251  &   $-$15.04  &   $<-$15.34  &   $-$15.28  &   $-$15.15  &     $-$14.89  &    $-$15.64  &   $-$14.60  &    $-$14.55  &    $-$14.83  &    $-$15.25  &    $-$15.29  &      1345  &        281  &       264  \\  %  53147-1676-530
252  &   $-$15.28  &    $-$14.19  &   $-$15.11  &   $-$14.39  &     $-$14.92  &    $-$15.78  &   $-$14.55  &    $-$13.94  &    $-$14.79  &    $-$15.35  &    $-$15.40  &       715  &        253  &       185  \\  %  53108-1385-233
253  &   $-$15.03  &    $-$14.15  &   $-$15.61  &   $-$14.24  &     $-$14.28  &    $-$15.60  &   $-$14.73  &    $-$13.68  &    $-$14.73  &    $-$15.29  &    $-$15.37  &      1013  &        254  &       251  \\  %  52703-1165-424
254  &   $-$14.70  &    $-$15.17  &   $-$15.16  &   $-$15.01  &     $-$14.82  &    $-$15.69  &   $-$14.51  &    $-$14.23  &    $-$15.11  &    $-$15.22  &    $-$15.40  &      1362  &        248  &       203  \\  %  52426-0922-589
255  &   $-$15.61  &    $-$14.83  &  $<-$15.98  &   $-$14.89  &     $-$15.72  &   $<-$16.13  &  $<-$15.53  &    $-$14.35  &    $-$15.60  &    $-$16.04  &    $-$16.06  &       633  &    \nodata  &       212  \\  %  52057-0590-103
256  &   $-$14.66  &    $-$14.69  &   $-$15.01  &   $-$14.48  &     $-$14.01  &    $-$15.33  &   $-$14.44  &    $-$13.95  &    $-$14.49  &    $-$15.00  &    $-$15.01  &       915  &        234  &       210  \\  %  53116-1386-550
257  &   $-$15.32  &    $-$14.25  &   $-$15.97  &   $-$14.59  &     $-$14.97  &    $-$15.73  &   $-$15.35  &    $-$14.07  &    $-$15.11  &    $-$15.62  &    $-$15.57  &       752  &        560  &       429  \\  %  52765-1293-387
258  &  $<-$15.58  &   $<-$15.18  &  $<-$15.78  &   $-$15.35  &     $-$15.51  &   $<-$16.05  &   $-$15.09  &    $-$14.80  &    $-$15.50  &    $-$15.97  &    $-$15.98  &      1152  &        199  &       280  \\  %  52736-1292-026
259  &   $-$15.82  &    $-$15.42  &   $-$16.40  &   $-$15.42  &     $-$15.29  &   $<-$16.03  &   $-$15.78  &    $-$14.78  &    $-$15.67  &    $-$16.38  &    $-$16.23  &       589  &        416  &   \nodata  \\  %  52376-0794-550
260  &   $-$14.18  &   $<-$15.03  &   $-$14.66  &   $-$14.27  &     $-$14.31  &    $-$15.33  &   $-$14.14  &    $-$13.73  &    $-$14.49  &    $-$14.76  &    $-$14.89  &      1277  &        192  &       154  \\  %  52411-0925-266
261  &   $-$15.57  &    $-$15.09  &   $-$15.72  &   $-$15.14  &     $-$15.17  &   $<-$16.15  &   $-$15.31  &    $-$14.62  &    $-$15.91  &    $-$16.04  &    $-$16.14  &       486  &         95  &        72  \\  %  52026-0593-547
262  &   $-$13.84  &   $<-$15.26  &   $-$14.20  &   $-$15.40  &     $-$13.59  &    $-$15.32  &   $-$13.68  &    $-$14.34  &    $-$14.86  &    $-$14.69  &    $-$14.85  &      1383  &        111  &       132  \\  %  53119-1388-039
263  &   $-$14.94  &    $-$14.59  &   $-$14.96  &   $-$14.58  &     $-$14.33  &    $-$15.54  &   $-$14.45  &    $-$13.90  &    $-$14.59  &    $-$15.13  &    $-$15.22  &      1089  &        210  &       249  \\  %  53135-1389-611
264  &   $-$15.17  &    $-$14.47  &   $-$15.27  &   $-$14.40  &     $-$14.46  &    $-$15.41  &   $-$14.49  &    $-$13.77  &    $-$14.90  &    $-$15.38  &    $-$15.45  &      1009  &        800  &       280  \\  %  52045-0594-216
265  &   $-$15.03  &    $-$14.90  &   $-$15.39  &   $-$14.93  &     $-$15.29  &   $<-$16.00  &   $-$14.88  &    $-$14.43  &    $-$15.20  &    $-$15.52  &    $-$15.77  &      1157  &        146  &       134  \\  %  52731-1168-417
266  &   $-$16.21  &    $-$15.29  &  $<-$16.20  &   $-$14.73  &     $-$15.13  &   $<-$15.97  &   $-$15.87  &    $-$14.13  &    $-$16.03  &   $<-$16.02  &   $<-$15.93  &       923  &        140  &   \nodata  \\  %  52782-1333-153
267  &   $-$14.97  &    $-$15.32  &   $-$15.28  &   $-$15.42  &     $-$14.28  &    $-$15.61  &   $-$14.74  &    $-$14.70  &    $-$14.81  &    $-$15.33  &    $-$15.33  &       562  &        182  &       165  \\  %  52516-1054-128
268  &   $-$15.18  &    $-$15.09  &   $-$15.48  &   $-$14.96  &     $-$14.73  &    $-$15.73  &   $-$14.78  &    $-$14.27  &    $-$14.89  &    $-$15.41  &    $-$15.40  &      1329  &        226  &       188  \\  %  52761-1055-086
269  &   $-$15.30  &    $-$14.12  &   $-$15.42  &   $-$14.37  &     $-$14.51  &   $<-$16.05  &   $-$14.74  &    $-$13.95  &    $-$14.84  &    $-$15.42  &    $-$15.54  &      1045  &        253  &       285  \\  %  51690-0345-601
270  &   $-$14.86  &   $<-$15.29  &   $-$15.17  &   $-$15.11  &     $-$14.81  &    $-$15.77  &   $-$14.52  &    $-$14.48  &    $-$14.85  &    $-$15.21  &    $-$15.37  &      1087  &        167  &       192  \\  %  51693-0346-147
271  &   $-$14.88  &    $-$13.98  &   $-$14.76  &   $-$14.00  &     $-$14.20  &    $-$15.34  &   $-$14.19  &    $-$13.49  &    $-$14.60  &    $-$15.24  &    $-$15.41  &       917  &        134  &       155  \\  %  52764-1056-067
272  &   $-$15.17  &   $<-$15.14  &   $-$15.95  &   $-$15.02  &     $-$15.18  &    $-$15.87  &   $-$15.33  &    $-$14.56  &    $-$14.96  &    $-$15.44  &    $-$15.51  &      2382  &        283  &       246  \\  %  52759-1172-346
273  &   $-$14.86  &    $-$14.42  &   $-$14.87  &   $-$14.47  &     $-$14.44  &    $-$15.52  &   $-$14.24  &    $-$13.86  &    $-$14.50  &    $-$15.12  &    $-$15.12  &       980  &        419  &       256  \\  %  53146-1420-093
274  &   $-$15.03  &   $<-$15.39  &   $-$15.23  &   $-$14.98  &     $-$14.55  &    $-$15.78  &   $-$14.70  &    $-$14.42  &    $-$14.88  &    $-$15.26  &    $-$15.32  &      1298  &        160  &       191  \\  %  52000-0364-259
275  &   $-$15.09  &    $-$15.14  &   $-$15.47  &   $-$14.87  &     $-$14.75  &    $-$15.77  &   $-$14.78  &    $-$14.31  &    $-$14.93  &    $-$15.38  &    $-$15.48  &       857  &        346  &       232  \\  %  52000-0364-128
276  &   $-$15.29  &   $<-$15.22  &   $-$15.38  &   $-$14.54  &     $-$14.85  &   $<-$15.95  &   $-$14.65  &    $-$14.04  &    $-$14.96  &    $-$15.42  &    $-$15.70  &       651  &        166  &       104  \\  %  52522-1057-630
277  &   $-$15.64  &    $-$14.79  &   $-$15.86  &   $-$14.99  &     $-$15.03  &    $-$15.96  &   $-$15.23  &    $-$14.44  &    $-$15.50  &    $-$15.87  &    $-$15.84  &       846  &        493  &       167  \\  %  52057-0626-433
278  &   $-$14.44  &    $-$14.89  &   $-$15.23  &   $-$14.37  &     $-$14.00  &    $-$15.43  &   $-$14.57  &    $-$13.78  &    $-$14.81  &    $-$14.98  &    $-$15.10  &       799  &        233  &       216  \\  %  53177-1572-457
279  &   $-$15.51  &    $-$14.74  &   $-$15.57  &   $-$15.01  &     $-$15.34  &    $-$16.26  &   $-$15.08  &    $-$14.36  &    $-$15.64  &    $-$15.78  &    $-$16.00  &       940  &        227  &       155  \\  %  52144-0627-631
280  &   $-$15.98  &   $<-$15.52  &   $-$16.04  &   $-$15.84  &     $-$15.80  &   $<-$16.03  &   $-$15.37  &    $-$15.28  &    $-$15.72  &    $-$16.22  &    $-$16.39  &       709  &    \nodata  &   \nodata  \\  %  52144-0627-604
281  &   $-$15.52  &   $<-$15.47  &   $-$16.05  &   $-$15.63  &     $-$15.67  &     \nodata  &   $-$15.61  &    $-$14.73  &     \nodata  &    $-$16.24  &   $<-$16.51  &      1489  &         85  &   \nodata  \\  %  52912-1424-260
282  &   $-$15.44  &    $-$14.81  &   $-$15.67  &   $-$14.96  &     $-$15.22  &    $-$16.19  &   $-$15.15  &    $-$14.40  &    $-$15.36  &    $-$15.79  &    $-$15.93  &       995  &        322  &       237  \\  %  51699-0349-364
283  &   $-$15.42  &    $-$14.97  &  $<-$15.77  &   $-$14.81  &     $-$14.76  &    $-$16.02  &  $<-$15.37  &    $-$14.20  &    $-$15.14  &    $-$15.63  &    $-$15.72  &       875  &        375  &       408  \\  %  51703-0353-460
284  &   $-$14.80  &    $-$15.04  &   $-$15.37  &   $-$14.65  &     $-$14.51  &    $-$15.28  &   $-$14.68  &    $-$14.16  &    $-$15.19  &    $-$15.30  &    $-$15.30  &       933  &        303  &       406  \\  %  51691-0350-263
285  &   $-$15.09  &   $<-$15.66  &   $-$15.37  &   $-$15.42  &     $-$15.05  &    $-$16.26  &   $-$14.83  &    $-$14.82  &    $-$15.20  &    $-$15.40  &    $-$15.54  &      1218  &        174  &       241  \\  %  51997-0367-298
286  &   $-$15.45  &    $-$15.23  &   $-$15.82  &   $-$15.29  &     $-$14.90  &    $-$15.78  &   $-$15.13  &    $-$14.65  &    $-$15.25  &    $-$15.89  &    $-$15.86  &      1000  &        496  &       273  \\  %  51788-0355-585
287  &   $-$15.13  &    $-$14.77  &   $-$15.39  &   $-$14.76  &     $-$14.52  &    $-$16.00  &   $-$14.89  &    $-$14.31  &    $-$15.35  &    $-$15.71  &    $-$15.79  &       835  &        175  &       183  \\  %  51821-0359-535
288  &   $-$14.65  &   $<-$15.31  &   $-$15.02  &   $-$14.91  &     $-$14.85  &    $-$15.94  &   $-$14.41  &    $-$14.45  &    $-$14.75  &    $-$15.26  &    $-$15.32  &       731  &        216  &       130  \\  %  52443-0983-382
289  &   $-$14.59  &    $-$14.37  &   $-$14.87  &   $-$14.20  &     $-$13.95  &    $-$15.43  &   $-$14.27  &    $-$13.73  &    $-$14.75  &    $-$15.06  &    $-$15.10  &       968  &        260  &       218  \\  %  52176-0636-105
290  &   $-$15.06  &    $-$15.03  &   $-$15.67  &   $-$14.85  &     $-$14.77  &    $-$15.61  &   $-$15.01  &    $-$14.25  &    $-$15.12  &    $-$15.42  &    $-$15.52  &      1402  &        296  &       230  \\  %  52431-0985-396
291  &   $-$15.61  &   $<-$15.38  &   $-$15.88  &    \nodata  &     $-$15.19  &   $<-$16.04  &   $-$15.28  &    $-$14.90  &    $-$15.29  &    $-$15.68  &    $-$15.89  &       695  &        205  &       238  \\  %  52520-0728-179
292  &   $-$15.23  &   $<-$15.29  &   $-$15.68  &   $-$15.25  &     $-$15.00  &   $<-$16.07  &   $-$15.04  &    $-$14.56  &    $-$15.21  &    $-$15.65  &    $-$15.65  &      1585  &        197  &       249  \\  %  52520-0728-563
293  &   $-$15.43  &   $<-$15.35  &   $-$15.93  &   $-$15.24  &     $-$14.97  &   $<-$16.06  &   $-$15.30  &    $-$14.68  &    $-$15.56  &    $-$16.04  &    $-$16.04  &      1350  &        251  &       237  \\  %  52178-0640-252
294  &   $-$15.08  &   $<-$15.42  &   $-$15.29  &  $<-$15.83  &     $-$14.36  &    $-$15.49  &   $-$14.79  &    $-$14.79  &    $-$14.96  &    $-$15.34  &    $-$15.44  &      1660  &        351  &       204  \\  %  52199-0641-531
295  &   $-$15.50  &   $<-$15.23  &   $-$15.56  &   $-$15.37  &     $-$15.33  &   $<-$16.07  &   $-$15.03  &    $-$14.70  &    $-$15.31  &    $-$15.85  &    $-$15.81  &      1008  &        190  &       158  \\  %  51791-0374-287
296  &   $-$15.25  &   $<-$15.45  &   $-$15.35  &   $-$15.27  &     $-$15.02  &    $-$16.20  &   $-$14.75  &    $-$14.79  &    $-$15.04  &    $-$15.50  &    $-$15.61  &       972  &        211  &       152  \\  %  52206-0718-608
297  &   $-$15.05  &    $-$14.84  &   $-$15.29  &   $-$14.71  &     $-$15.00  &    $-$15.51  &   $-$14.69  &    $-$14.13  &    $-$14.99  &    $-$15.39  &    $-$15.50  &       791  &        236  &       211  \\  %  52520-0739-416
298  &   $-$15.22  &    $-$14.92  &   $-$15.36  &   $-$15.06  &     $-$14.93  &    $-$16.07  &   $-$14.78  &    $-$14.56  &    $-$15.20  &    $-$15.53  &    $-$15.54  &      1154  &        260  &       281  \\  %  52263-0742-353
299  &   $-$14.90  &   $<-$15.25  &   $-$15.03  &   $-$15.07  &     $-$14.52  &    $-$15.78  &   $-$14.45  &    $-$14.33  &    $-$14.67  &    $-$15.15  &    $-$15.26  &      1546  &        161  &       149  \\  %  51811-0381-363
300  &  $<-$15.41  &   $<-$15.11  &   $-$15.77  &   $-$15.44  &     $-$15.33  &   $<-$16.05  &   $-$14.83  &    $-$14.70  &    $-$15.15  &    $-$15.59  &    $-$15.60  &      1573  &        290  &       311  \\  %  52262-0743-506
301  &   $-$15.62  &    $-$15.34  &   $-$15.82  &   $-$15.49  &     $-$15.15  &   $<-$16.25  &   $-$15.20  &    $-$15.13  &    $-$15.60  &    $-$16.09  &   $<-$16.32  &      1245  &        275  &       236  \\  %  52226-0726-257
302  &   $-$15.70  &    $-$14.79  &   $-$16.17  &   $-$14.82  &     $-$15.21  &     \nodata  &   $-$15.55  &    $-$14.28  &    $-$15.52  &    $-$15.93  &   $<-$16.18  &       806  &        330  &       153  \\  %  52523-0646-560
303  &   $-$14.61  &   $<-$15.48  &   $-$15.05  &   $-$15.57  &     $-$13.87  &    $-$15.26  &   $-$14.48  &    $-$14.60  &    $-$14.56  &    $-$14.94  &    $-$14.95  &       980  &        147  &       156  \\  %  51877-0385-264
304  &   $-$15.32  &    $-$14.66  &   $-$15.72  &   $-$14.72  &     $-$14.82  &    $-$15.80  &   $-$14.91  &    $-$14.20  &    $-$15.06  &    $-$15.48  &    $-$15.64  &       946  &        221  &        90  \\  %  51877-0385-379
305  &   $-$14.97  &   $<-$15.46  &   $-$15.25  &  $<-$15.95  &     $-$14.30  &    $-$15.73  &   $-$14.55  &    $-$14.42  &    $-$14.70  &    $-$15.17  &    $-$15.27  &      1144  &        274  &       229  \\  %  51877-0385-121
306  &   $-$15.01  &   $<-$15.38  &   $-$15.18  &   $-$15.71  &     $-$15.12  &    $-$15.70  &   $-$14.45  &    $-$14.60  &    $-$14.74  &    $-$15.14  &    $-$15.23  &      1409  &        379  &       222  \\  %  52559-0648-572
307  &   $-$15.33  &   $<-$15.48  &   $-$15.42  &   $-$15.23  &     $-$15.26  &    $-$16.12  &   $-$14.87  &    $-$14.64  &    $-$15.25  &    $-$15.72  &    $-$15.88  &      1103  &        248  &       240  \\  %  52226-0749-439
308  &   $-$14.98  &   $<-$15.27  &   $-$15.41  &  $<-$15.63  &     $-$14.87  &    $-$15.57  &   $-$14.81  &    $-$14.80  &    $-$14.96  &    $-$15.31  &    $-$15.42  &      1573  &        323  &       175  \\  %  51788-0386-197
309  &   $-$15.51  &   $<-$15.40  &   $-$16.11  &   $-$15.19  &     $-$15.13  &   $<-$15.81  &   $-$15.23  &    $-$14.73  &    $-$15.46  &    $-$15.78  &    $-$16.06  &      1320  &        272  &       164      %  51791-0387-432


==> full_table3.tex <==
%% ID&   TOTAL    &     AGN    &    HOST    &   LBHA  &  MBH  &   ELL        %  SPEC
1    &  $-$18.30  &  $-$15.65  &  $-$18.20  &  40.04  &  6.2  &  $-$1.6  \\  %  52143-0650-174
2    &  $-$20.66  &  $-$17.23  &  $-$20.61  &  40.77  &  5.9  &  $-$0.6  \\  %  52235-0750-609
3    &  $-$21.06  &  $-$17.47  &  $-$21.02  &  40.89  &  6.0  &  $-$0.7  \\  %  51795-0389-120
4    &  $-$20.98  &  $-$18.26  &  $-$20.89  &  41.25  &  6.2  &  $-$0.6  \\  %  51900-0390-624
5    &  $-$20.66  &  $-$17.12  &  $-$20.62  &  40.72  &  6.2  &  $-$1.0  \\  %  51821-0417-182
6    &  $-$17.92  &  $-$14.56  &  $-$17.87  &  39.54  &  6.1  &  $-$1.9  \\  %  52162-0655-089
7    &  $-$18.47  &  $-$16.66  &  $-$18.24  &  40.51  &  5.6  &  $-$0.7  \\  %  51913-0394-624
8    &  $-$20.12  &  $-$18.27  &  $-$19.91  &  41.25  &  6.3  &  $-$0.7  \\  %  52146-0658-488
9    &  $-$20.77  &  $-$19.34  &  $-$20.43  &  41.75  &  6.0  &  $ $0.0  \\  %  51811-0422-321
10   &  $-$19.60  &  $-$18.26  &  $-$19.22  &  41.25  &  6.1  &  $-$0.5  \\  %  51811-0422-224
11   &  $-$20.10  &  $-$18.52  &  $-$19.81  &  41.37  &  5.7  &  $-$0.0  \\  %  52177-0660-142
12   &  $-$20.18  &  $-$18.15  &  $-$20.00  &  41.20  &  6.3  &  $-$0.7  \\  %  51817-0399-317
13   &  $-$20.55  &  $-$17.61  &  $-$20.47  &  40.95  &  6.3  &  $-$0.9  \\  %  52163-0661-229
14   &  $-$21.68  &  $-$20.26  &  $-$21.34  &  42.18  &  6.3  &  $ $0.1  \\  %  51893-0424-097
15   &  $-$19.76  &  $-$18.39  &  $-$19.39  &  41.31  &  5.9  &  $-$0.2  \\  %  51820-0429-084
16   &  $-$20.12  &  $-$15.29  &  $-$20.11  &  39.87  &  6.2  &  $-$1.7  \\  %  51900-0427-492
17   &  $-$20.33  &  $-$18.68  &  $-$20.06  &  41.45  &  6.1  &  $-$0.4  \\  %  51820-0407-329
18   &  $-$19.51  &  $-$16.50  &  $-$19.44  &  40.44  &  5.4  &  $-$0.5  \\  %  51908-0454-109
19   &  $-$20.67  &  $-$18.33  &  $-$20.53  &  41.28  &  6.1  &  $-$0.5  \\  %  51910-0456-257
20   &  $-$19.17  &  $-$15.53  &  $-$19.14  &  39.99  &  5.4  &  $-$0.9  \\  %  51910-0456-077
21   &  $-$20.95  &  $-$18.20  &  $-$20.86  &  41.22  &  6.2  &  $-$0.6  \\  %  51817-0411-513
22   &  $-$20.41  &  $-$17.14  &  $-$20.36  &  40.73  &  6.0  &  $-$0.9  \\  %  51929-0413-470
23   &  $-$19.53  &  $-$18.05  &  $-$19.21  &  41.15  &  5.9  &  $-$0.4  \\  %  51901-0414-405
24   &  $-$21.66  &  $-$19.31  &  $-$21.53  &  41.74  &  6.3  &  $-$0.3  \\  %  51901-0414-426
25   &  $-$20.27  &  $-$16.81  &  $-$20.22  &  40.58  &  6.0  &  $-$1.0  \\  %  51924-0460-014
26   &  $-$21.34  &  $-$19.53  &  $-$21.12  &  41.84  &  6.2  &  $-$0.1  \\  %  51909-0462-504
27   &  $-$20.74  &  $-$17.53  &  $-$20.68  &  40.91  &  6.0  &  $-$0.7  \\  %  53034-1734-137
28   &  $-$20.28  &  $-$17.23  &  $-$20.22  &  40.77  &  6.2  &  $-$1.0  \\  %  51877-0431-533
29   &  $-$19.73  &  $-$16.02  &  $-$19.69  &  40.21  &  6.1  &  $-$1.3  \\  %  51884-0432-384
30   &  $-$20.29  &  $-$17.94  &  $-$20.16  &  41.10  &  6.0  &  $-$0.5  \\  %  51959-0541-617
31   &  $-$21.25  &  $-$16.30  &  $-$21.24  &  40.34  &  5.9  &  $-$1.1  \\  %  52314-0857-039
32   &  $-$20.28  &  $-$16.84  &  $-$20.23  &  40.59  &  6.3  &  $-$1.2  \\  %  51959-0541-602
33   &  $-$21.23  &  $-$18.14  &  $-$21.17  &  41.19  &  6.3  &  $-$0.7  \\  %  53052-1736-062
34   &  $-$21.70  &  $-$16.86  &  $-$21.69  &  40.60  &  6.3  &  $-$1.2  \\  %  53055-1737-220
35   &  $-$18.76  &  $-$18.22  &  $-$17.73  &  41.23  &  6.3  &  $-$0.7  \\  %  53055-1737-468
36   &  $-$20.87  &  $-$18.38  &  $-$20.76  &  41.31  &  6.0  &  $-$0.4  \\  %  52316-0858-438
37   &  $-$20.57  &  $-$15.90  &  $-$20.56  &  40.16  &  6.0  &  $-$1.3  \\  %  52583-0890-400
38   &  $-$20.61  &  $-$16.67  &  $-$20.58  &  40.51  &  6.2  &  $-$1.2  \\  %  51869-0437-274
39   &  $-$19.97  &  $-$16.33  &  $-$19.93  &  40.36  &  5.8  &  $-$0.9  \\  %  53090-1780-369
40   &  $-$20.54  &  $-$15.90  &  $-$20.53  &  40.16  &  5.9  &  $-$1.3  \\  %  52670-1205-330
41   &  $-$19.90  &  $-$18.97  &  $-$19.31  &  41.58  &  6.2  &  $-$0.3  \\  %  53080-1756-305
42   &  $-$20.94  &  $-$16.68  &  $-$20.91  &  40.52  &  6.1  &  $-$1.1  \\  %  52253-0758-109
43   &  $-$20.12  &  $-$16.61  &  $-$20.07  &  40.49  &  5.8  &  $-$0.8  \\  %  52705-1265-139
44   &  $-$20.56  &  $-$17.13  &  $-$20.51  &  40.73  &  6.1  &  $-$0.9  \\  %  52378-0892-244
45   &  $-$19.39  &  $-$16.83  &  $-$19.29  &  40.59  &  5.8  &  $-$0.8  \\  %  51877-0439-216
46   &  $-$19.40  &  $-$16.45  &  $-$19.33  &  40.41  &  6.0  &  $-$1.1  \\  %  52318-0861-430
47   &  $-$20.12  &  $-$18.00  &  $-$19.96  &  41.13  &  5.9  &  $-$0.4  \\  %  52325-0862-287
48   &  $-$19.89  &  $-$16.47  &  $-$19.85  &  40.42  &  5.9  &  $-$1.0  \\  %  52709-1266-109
49   &  $-$18.91  &  $-$15.23  &  $-$18.87  &  39.85  &  6.0  &  $-$1.6  \\  %  51868-0441-438
50   &  $-$21.27  &  $-$18.05  &  $-$21.21  &  41.15  &  6.0  &  $-$0.5  \\  %  51868-0441-106
51   &  $-$19.96  &  $-$18.63  &  $-$19.59  &  41.42  &  6.3  &  $-$0.5  \\  %  52962-1585-549
52   &  $-$20.77  &  $-$15.55  &  $-$20.76  &  40.00  &  5.9  &  $-$1.4  \\  %  52962-1296-371
53   &  $-$21.58  &  $-$18.94  &  $-$21.48  &  41.56  &  6.0  &  $-$0.1  \\  %  51882-0442-420
54   &  $-$21.73  &  $-$18.54  &  $-$21.67  &  41.38  &  6.1  &  $-$0.4  \\  %  52589-0893-636
55   &  $-$19.68  &  $-$16.70  &  $-$19.61  &  40.53  &  6.1  &  $-$1.1  \\  %  53084-1758-332
56   &  $-$21.09  &  $-$17.91  &  $-$21.03  &  41.09  &  5.5  &  $-$0.0  \\  %  52932-1267-107
57   &  $-$18.90  &  $-$17.78  &  $-$18.43  &  41.03  &  5.9  &  $-$0.5  \\  %  51873-0443-514
58   &  $-$20.62  &  $-$15.65  &  $-$20.61  &  40.04  &  6.1  &  $-$1.5  \\  %  53084-1758-524
59   &  $-$20.05  &  $-$17.92  &  $-$19.89  &  41.09  &  5.8  &  $-$0.3  \\  %  51873-0445-301
60   &  $-$20.64  &  $-$17.28  &  $-$20.59  &  40.79  &  5.8  &  $-$0.6  \\  %  52963-1297-154
61   &  $-$17.72  &  $-$14.75  &  $-$17.65  &  39.63  &  6.1  &  $-$1.9  \\  %  51899-0446-271
62   &  $-$20.91  &  $-$19.03  &  $-$20.70  &  41.60  &  6.3  &  $-$0.3  \\  %  53081-1759-148
63   &  $-$20.97  &  $-$17.91  &  $-$20.90  &  41.09  &  5.9  &  $-$0.4  \\  %  52964-1298-335
64   &  $-$21.02  &  $-$15.53  &  $-$21.01  &  39.99  &  5.9  &  $-$1.3  \\  %  52320-0864-067
65   &  $-$21.12  &  $-$19.82  &  $-$20.72  &  41.97  &  6.2  &  $ $0.1  \\  %  52323-0865-191
66   &  $-$20.36  &  $-$17.17  &  $-$20.30  &  40.74  &  6.1  &  $-$0.9  \\  %  52672-0934-517
67   &  $-$21.10  &  $-$17.19  &  $-$21.07  &  40.76  &  5.8  &  $-$0.6  \\  %  51877-0447-554
68   &  $-$21.15  &  $-$18.63  &  $-$21.04  &  41.42  &  6.3  &  $-$0.5  \\  %  52293-0830-239
69   &  $-$21.21  &  $-$18.92  &  $-$21.07  &  41.56  &  6.0  &  $-$0.2  \\  %  52605-0897-178
70   &  $-$21.16  &  $-$18.72  &  $-$21.03  &  41.46  &  6.0  &  $-$0.2  \\  %  52964-1211-420
71   &  $-$20.56  &  $-$17.62  &  $-$20.48  &  40.95  &  5.5  &  $-$0.2  \\  %  51900-0449-571
72   &  $-$19.68  &  $-$15.81  &  $-$19.65  &  40.12  &  6.1  &  $-$1.5  \\  %  52294-0831-464
73   &  $-$19.40  &  $-$18.40  &  $-$18.85  &  41.32  &  6.1  &  $-$0.4  \\  %  52649-1192-183
74   &  $-$19.97  &  $-$18.21  &  $-$19.73  &  41.23  &  6.0  &  $-$0.4  \\  %  52973-1300-127
75   &  $-$19.25  &  $-$17.31  &  $-$19.05  &  40.81  &  5.8  &  $-$0.6  \\  %  52312-0832-397
76   &  $-$19.69  &  $-$18.04  &  $-$19.43  &  41.15  &  6.2  &  $-$0.7  \\  %  52620-0899-367
77   &  $-$19.07  &  $-$15.60  &  $-$19.02  &  40.02  &  5.9  &  $-$1.3  \\  %  51908-0450-108
78   &  $-$20.80  &  $-$18.82  &  $-$20.61  &  41.51  &  6.3  &  $-$0.4  \\  %  52976-1301-471
79   &  $-$21.85  &  $-$20.30  &  $-$21.56  &  42.19  &  6.3  &  $ $0.1  \\  %  52652-1193-563
80   &  $-$20.71  &  $-$18.87  &  $-$20.50  &  41.53  &  5.7  &  $ $0.2  \\  %  52707-0937-066
81   &  $-$21.39  &  $-$19.46  &  $-$21.19  &  41.81  &  6.2  &  $-$0.1  \\  %  52707-0991-391
82   &  $-$21.55  &  $-$17.27  &  $-$21.53  &  40.79  &  6.1  &  $-$0.9  \\  %  52707-0991-268
83   &  $-$20.74  &  $-$15.65  &  $-$20.73  &  40.04  &  6.1  &  $-$1.5  \\  %  52000-0474-225
84   &  $-$20.86  &  $-$16.04  &  $-$20.85  &  40.22  &  6.2  &  $-$1.4  \\  %  51929-0473-619
85   &  $-$19.76  &  $-$18.57  &  $-$19.31  &  41.39  &  5.6  &  $ $0.1  \\  %  52707-0991-061
86   &  $-$20.42  &  $-$18.42  &  $-$20.23  &  41.32  &  6.3  &  $-$0.6  \\  %  53050-1303-300
87   &  $-$20.10  &  $-$17.88  &  $-$19.95  &  41.07  &  5.9  &  $-$0.4  \\  %  52266-0555-049
88   &  $-$20.28  &  $-$18.28  &  $-$20.09  &  41.26  &  6.3  &  $-$0.7  \\  %  51915-0453-310
89   &  $-$20.20  &  $-$17.85  &  $-$20.07  &  41.06  &  6.0  &  $-$0.5  \\  %  52264-0569-634
90   &  $-$19.86  &  $-$16.81  &  $-$19.79  &  40.58  &  5.7  &  $-$0.7  \\  %  52725-1215-114
91   &  $-$21.20  &  $-$18.80  &  $-$21.08  &  41.50  &  6.1  &  $-$0.2  \\  %  52724-1234-390
92   &  $-$19.50  &  $-$17.77  &  $-$19.25  &  41.02  &  6.1  &  $-$0.7  \\  %  51910-0486-059
93   &  $-$18.61  &  $-$16.14  &  $-$18.50  &  40.27  &  6.2  &  $-$1.5  \\  %  52757-1305-179
94   &  $-$20.05  &  $-$15.94  &  $-$20.03  &  40.18  &  6.3  &  $-$1.6  \\  %  51943-0487-424
95   &  $-$20.13  &  $-$16.99  &  $-$20.07  &  40.66  &  6.2  &  $-$1.0  \\  %  52725-0994-490
96   &  $-$20.24  &  $-$15.30  &  $-$20.22  &  39.88  &  5.9  &  $-$1.5  \\  %  52998-1596-344
97   &  $-$19.62  &  $-$16.74  &  $-$19.54  &  40.55  &  6.0  &  $-$1.0  \\  %  52317-0558-282
98   &  $-$18.92  &  $-$18.50  &  $-$17.69  &  41.36  &  6.2  &  $-$0.5  \\  %  52709-1216-120
99   &  $-$20.92  &  $-$19.41  &  $-$20.60  &  41.78  &  6.0  &  $ $0.1  \\  %  52282-0769-062
100  &  $-$20.75  &  $-$18.44  &  $-$20.61  &  41.33  &  6.3  &  $-$0.6  \\  %  51633-0268-085
101  &  $-$19.29  &  $-$16.02  &  $-$19.23  &  40.21  &  5.3  &  $-$0.6  \\  %  52652-0945-172
102  &  $-$19.81  &  $-$18.31  &  $-$19.49  &  41.27  &  5.9  &  $-$0.2  \\  %  52993-1426-132
103  &  $-$20.68  &  $-$19.10  &  $-$20.39  &  41.64  &  6.2  &  $-$0.2  \\  %  52317-0558-611
104  &  $-$19.25  &  $-$18.09  &  $-$18.79  &  41.17  &  5.9  &  $-$0.4  \\  %  51909-0270-490
105  &  $-$19.17  &  $-$17.43  &  $-$18.92  &  40.87  &  6.1  &  $-$0.8  \\  %  51883-0271-277
106  &  $-$20.08  &  $-$18.84  &  $-$19.67  &  41.52  &  5.8  &  $ $0.0  \\  %  53034-1357-543
107  &  $-$20.52  &  $-$15.55  &  $-$20.51  &  40.00  &  6.0  &  $-$1.5  \\  %  51999-0503-098
108  &  $-$18.77  &  $-$15.13  &  $-$18.73  &  39.80  &  5.8  &  $-$1.5  \\  %  52998-1428-232
109  &  $-$19.72  &  $-$16.89  &  $-$19.64  &  40.62  &  6.3  &  $-$1.2  \\  %  51999-0503-585
110  &  $-$21.22  &  $-$16.56  &  $-$21.21  &  40.46  &  5.4  &  $-$0.5  \\  %  52319-0575-199
111  &  $-$21.37  &  $-$17.15  &  $-$21.34  &  40.74  &  6.0  &  $-$0.9  \\  %  52338-0874-499
112  &  $-$18.59  &  $-$12.31  &  $-$18.58  &  38.50  &  5.7  &  $-$2.4  \\  %  51930-0489-193
113  &  $-$19.86  &  $-$18.17  &  $-$19.61  &  41.21  &  6.1  &  $-$0.5  \\  %  53089-1599-555
114  &  $-$20.43  &  $-$18.28  &  $-$20.27  &  41.26  &  6.3  &  $-$0.6  \\  %  52367-0577-414
115  &  $-$21.48  &  $-$16.14  &  $-$21.47  &  40.27  &  6.0  &  $-$1.2  \\  %  52376-0773-258
116  &  $-$18.91  &  $-$17.12  &  $-$18.68  &  40.72  &  6.3  &  $-$1.1  \\  %  52428-0948-259
117  &  $-$20.11  &  $-$18.67  &  $-$19.78  &  41.44  &  6.1  &  $-$0.3  \\  %  51910-0275-312
118  &  $-$20.25  &  $-$17.83  &  $-$20.13  &  41.05  &  6.2  &  $-$0.8  \\  %  53115-1601-427
119  &  $-$20.44  &  $-$15.50  &  $-$20.42  &  39.97  &  6.0  &  $-$1.5  \\  %  53047-1361-020
120  &  $-$20.26  &  $-$18.17  &  $-$20.09  &  41.21  &  6.1  &  $-$0.5  \\  %  52669-0876-497
121  &  $-$20.11  &  $-$15.80  &  $-$20.09  &  40.11  &  5.3  &  $-$0.7  \\  %  53054-1436-303
122  &  $-$19.56  &  $-$16.80  &  $-$19.47  &  40.57  &  5.9  &  $-$0.9  \\  %  52643-0963-626
123  &  $-$22.39  &  $-$20.55  &  $-$22.17  &  42.31  &  6.2  &  $ $0.3  \\  %  52646-1002-117
124  &  $-$20.35  &  $-$16.26  &  $-$20.33  &  40.32  &  6.1  &  $-$1.2  \\  %  52723-1220-172
125  &  $-$21.63  &  $-$19.58  &  $-$21.45  &  41.86  &  6.0  &  $ $0.2  \\  %  53054-1436-523
126  &  $-$20.46  &  $-$19.01  &  $-$20.13  &  41.60  &  6.2  &  $-$0.3  \\  %  52751-1221-253
127  &  $-$21.15  &  $-$18.66  &  $-$21.03  &  41.43  &  6.0  &  $-$0.2  \\  %  52356-0581-254
128  &  $-$21.18  &  $-$19.46  &  $-$20.93  &  41.81  &  6.2  &  $-$0.1  \\  %  53078-1604-332
129  &  $-$21.19  &  $-$17.39  &  $-$21.16  &  40.85  &  6.1  &  $-$0.9  \\  %  51900-0278-279
130  &  $-$21.35  &  $-$18.53  &  $-$21.26  &  41.37  &  6.2  &  $-$0.5  \\  %  53078-1604-242
131  &  $-$20.20  &  $-$17.94  &  $-$20.06  &  41.10  &  6.1  &  $-$0.6  \\  %  52374-0509-143
132  &  $-$19.99  &  $-$18.12  &  $-$19.77  &  41.18  &  6.1  &  $-$0.5  \\  %  52374-0509-508
133  &  $-$19.53  &  $-$16.54  &  $-$19.46  &  40.45  &  6.3  &  $-$1.3  \\  %  53046-1437-636
134  &  $-$20.71  &  $-$17.00  &  $-$20.67  &  40.67  &  6.3  &  $-$1.2  \\  %  52646-0964-636
135  &  $-$20.62  &  $-$16.36  &  $-$20.60  &  40.37  &  6.0  &  $-$1.2  \\  %  52649-1012-401
136  &  $-$21.68  &  $-$20.17  &  $-$21.37  &  42.14  &  6.2  &  $ $0.1  \\  %  52381-0510-198
137  &  $-$20.77  &  $-$18.04  &  $-$20.68  &  41.15  &  6.2  &  $-$0.7  \\  %  52649-1012-133
138  &  $-$19.88  &  $-$17.90  &  $-$19.69  &  41.08  &  5.8  &  $-$0.4  \\  %  53084-1440-250
139  &  $-$20.65  &  $-$15.81  &  $-$20.64  &  40.12  &  5.9  &  $-$1.2  \\  %  52707-1013-169
140  &  $-$18.13  &  $-$16.47  &  $-$17.87  &  40.42  &  6.1  &  $-$1.2  \\  %  53084-1440-512
141  &  $-$20.06  &  $-$15.90  &  $-$20.04  &  40.16  &  6.2  &  $-$1.5  \\  %  52365-0879-328
142  &  $-$19.98  &  $-$18.27  &  $-$19.72  &  41.26  &  6.1  &  $-$0.4  \\  %  53062-1365-124
143  &  $-$20.16  &  $-$17.27  &  $-$20.09  &  40.79  &  6.1  &  $-$0.9  \\  %  52636-0511-031
144  &  $-$20.46  &  $-$17.30  &  $-$20.40  &  40.81  &  6.0  &  $-$0.7  \\  %  52781-1223-409
145  &  $-$18.70  &  $-$16.16  &  $-$18.59  &  40.28  &  6.3  &  $-$1.5  \\  %  53083-1441-619
146  &  $-$19.38  &  $-$15.53  &  $-$19.35  &  39.99  &  5.9  &  $-$1.4  \\  %  52365-0879-200
147  &  $-$18.89  &  $-$17.27  &  $-$18.61  &  40.79  &  5.7  &  $-$0.5  \\  %  53050-1442-263
148  &  $-$21.36  &  $-$16.80  &  $-$21.34  &  40.58  &  5.6  &  $-$0.5  \\  %  52409-0952-228
149  &  $-$21.02  &  $-$17.88  &  $-$20.96  &  41.07  &  6.2  &  $-$0.8  \\  %  52059-0597-560
150  &  $-$20.18  &  $-$17.87  &  $-$20.04  &  41.07  &  6.0  &  $-$0.6  \\  %  53055-1443-608
151  &  $-$19.43  &  $-$17.97  &  $-$19.11  &  41.12  &  6.3  &  $-$0.8  \\  %  53055-1443-009
152  &  $-$20.97  &  $-$15.63  &  $-$20.96  &  40.03  &  6.0  &  $-$1.5  \\  %  53083-1607-513
153  &  $-$20.68  &  $-$18.35  &  $-$20.55  &  41.29  &  5.7  &  $-$0.0  \\  %  51994-0514-331
154  &  $-$20.05  &  $-$15.43  &  $-$20.03  &  39.94  &  6.1  &  $-$1.6  \\  %  52282-0328-197
155  &  $-$21.96  &  $-$19.86  &  $-$21.79  &  41.99  &  6.1  &  $ $0.2  \\  %  53083-1367-481
156  &  $-$20.69  &  $-$19.85  &  $-$20.02  &  41.99  &  6.3  &  $-$0.0  \\  %  52316-0598-301
157  &  $-$20.12  &  $-$17.63  &  $-$20.00  &  40.96  &  6.1  &  $-$0.8  \\  %  52282-0328-107
158  &  $-$17.94  &  $-$15.83  &  $-$17.77  &  40.13  &  5.6  &  $-$1.0  \\  %  52734-1015-596
159  &  $-$21.15  &  $-$19.05  &  $-$20.98  &  41.62  &  6.3  &  $-$0.3  \\  %  53084-1368-285
160  &  $-$20.44  &  $-$18.44  &  $-$20.26  &  41.33  &  5.8  &  $-$0.1  \\  %  52734-1226-485
161  &  $-$21.25  &  $-$17.62  &  $-$21.21  &  40.95  &  6.2  &  $-$0.8  \\  %  52056-0329-169
162  &  $-$19.11  &  $-$16.77  &  $-$18.98  &  40.56  &  6.1  &  $-$1.1  \\  %  52367-0880-032
163  &  $-$19.63  &  $-$17.35  &  $-$19.49  &  40.83  &  6.1  &  $-$0.8  \\  %  52781-1312-121
164  &  $-$20.14  &  $-$18.10  &  $-$19.96  &  41.17  &  6.1  &  $-$0.5  \\  %  53080-1446-129
165  &  $-$20.93  &  $-$19.31  &  $-$20.66  &  41.74  &  6.1  &  $-$0.1  \\  %  52411-0953-077
166  &  $-$20.49  &  $-$16.92  &  $-$20.45  &  40.63  &  6.2  &  $-$1.1  \\  %  52442-0969-445
167  &  $-$20.94  &  $-$17.06  &  $-$20.91  &  40.70  &  6.2  &  $-$1.1  \\  %  52367-0332-604
168  &  $-$20.38  &  $-$15.28  &  $-$20.37  &  39.87  &  6.2  &  $-$1.7  \\  %  53090-1370-483
169  &  $-$19.73  &  $-$17.53  &  $-$19.57  &  40.91  &  5.9  &  $-$0.6  \\  %  52282-0518-218
170  &  $-$19.45  &  $-$16.18  &  $-$19.39  &  40.29  &  6.1  &  $-$1.3  \\  %  52409-0955-466
171  &  $-$21.50  &  $-$18.44  &  $-$21.43  &  41.34  &  6.2  &  $-$0.5  \\  %  52413-0970-558
172  &  $-$20.47  &  $-$16.19  &  $-$20.45  &  40.29  &  6.2  &  $-$1.4  \\  %  52430-0883-606
173  &  $-$20.21  &  $-$17.89  &  $-$20.07  &  41.08  &  6.3  &  $-$0.8  \\  %  52672-1230-131
174  &  $-$17.98  &  $-$15.77  &  $-$17.83  &  40.10  &  5.6  &  $-$0.9  \\  %  52791-1315-568
175  &  $-$20.91  &  $-$17.63  &  $-$20.85  &  40.96  &  5.6  &  $-$0.3  \\  %  53140-1625-071
176  &  $-$21.33  &  $-$17.03  &  $-$21.31  &  40.68  &  6.1  &  $-$1.0  \\  %  53112-1452-157
177  &  $-$18.61  &  $-$16.70  &  $-$18.41  &  40.53  &  5.6  &  $-$0.6  \\  %  52342-0779-621
178  &  $-$20.42  &  $-$16.34  &  $-$20.39  &  40.36  &  6.2  &  $-$1.3  \\  %  52317-0600-437
179  &  $-$19.64  &  $-$18.39  &  $-$19.23  &  41.31  &  5.6  &  $ $0.0  \\  %  51990-0289-625
180  &  $-$20.10  &  $-$18.63  &  $-$19.77  &  41.42  &  6.1  &  $-$0.3  \\  %  52317-0600-043
181  &  $-$20.01  &  $-$18.79  &  $-$19.59  &  41.49  &  6.1  &  $-$0.2  \\  %  51941-0290-021
182  &  $-$20.40  &  $-$16.42  &  $-$20.38  &  40.40  &  6.3  &  $-$1.4  \\  %  51928-0291-375
183  &  $-$20.35  &  $-$17.03  &  $-$20.30  &  40.68  &  6.2  &  $-$1.1  \\  %  52765-1317-421
184  &  $-$21.12  &  $-$19.82  &  $-$20.73  &  41.97  &  6.3  &  $-$0.0  \\  %  52379-0885-107
185  &  $-$20.17  &  $-$18.56  &  $-$19.89  &  41.39  &  5.9  &  $-$0.2  \\  %  52373-0781-076
186  &  $-$19.76  &  $-$17.92  &  $-$19.54  &  41.09  &  6.2  &  $-$0.7  \\  %  51997-0337-425
187  &  $-$20.15  &  $-$18.07  &  $-$19.98  &  41.16  &  5.7  &  $-$0.1  \\  %  52316-0601-533
188  &  $-$19.50  &  $-$16.15  &  $-$19.45  &  40.28  &  6.1  &  $-$1.3  \\  %  53116-1457-236
189  &  $-$20.01  &  $-$18.49  &  $-$19.71  &  41.36  &  6.2  &  $-$0.5  \\  %  52736-1279-075
190  &  $-$20.54  &  $-$16.40  &  $-$20.51  &  40.39  &  6.3  &  $-$1.4  \\  %  51994-0293-525
191  &  $-$21.46  &  $-$18.61  &  $-$21.38  &  41.41  &  5.8  &  $-$0.1  \\  %  51986-0294-296
192  &  $-$19.64  &  $-$17.27  &  $-$19.51  &  40.79  &  6.3  &  $-$1.0  \\  %  53083-1374-542
193  &  $-$19.41  &  $-$17.62  &  $-$19.18  &  40.96  &  6.2  &  $-$0.8  \\  %  52376-0887-100
194  &  $-$21.21  &  $-$19.27  &  $-$21.01  &  41.72  &  6.0  &  $ $0.0  \\  %  52027-0524-640
195  &  $-$21.92  &  $-$17.75  &  $-$21.90  &  41.02  &  5.9  &  $-$0.5  \\  %  52072-0602-051
196  &  $-$19.76  &  $-$16.98  &  $-$19.67  &  40.66  &  6.3  &  $-$1.2  \\  %  52295-0525-091
197  &  $-$19.40  &  $-$16.50  &  $-$19.32  &  40.44  &  5.4  &  $-$0.5  \\  %  52338-0850-585
198  &  $-$21.55  &  $-$19.35  &  $-$21.39  &  41.76  &  6.1  &  $-$0.1  \\  %  53142-1697-464
199  &  $-$20.06  &  $-$18.36  &  $-$19.80  &  41.30  &  6.0  &  $-$0.4  \\  %  53112-1773-411
200  &  $-$20.43  &  $-$19.38  &  $-$19.90  &  41.77  &  6.3  &  $-$0.2  \\  %  53112-1773-226
201  &  $-$20.20  &  $-$17.57  &  $-$20.10  &  40.93  &  6.2  &  $-$0.9  \\  %  52312-0526-309
202  &  $-$20.48  &  $-$18.36  &  $-$20.31  &  41.30  &  6.2  &  $-$0.5  \\  %  52759-1282-271
203  &  $-$21.61  &  $-$17.81  &  $-$21.57  &  41.04  &  6.3  &  $-$0.8  \\  %  53138-1460-004
204  &  $-$20.19  &  $-$18.01  &  $-$20.03  &  41.14  &  5.9  &  $-$0.4  \\  %  53146-1698-257
205  &  $-$19.88  &  $-$17.70  &  $-$19.72  &  40.99  &  5.6  &  $-$0.2  \\  %  53089-1376-087
206  &  $-$18.79  &  $-$15.01  &  $-$18.76  &  39.75  &  5.8  &  $-$1.4  \\  %  52375-0852-394
207  &  $-$19.90  &  $-$17.82  &  $-$19.73  &  41.05  &  6.0  &  $-$0.5  \\  %  51988-0496-091
208  &  $-$20.59  &  $-$17.73  &  $-$20.51  &  41.00  &  6.0  &  $-$0.6  \\  %  52426-0911-283
209  &  $-$21.37  &  $-$18.39  &  $-$21.30  &  41.31  &  5.8  &  $-$0.1  \\  %  52377-0910-144
210  &  $-$20.79  &  $-$17.79  &  $-$20.72  &  41.03  &  6.3  &  $-$0.9  \\  %  52022-0528-152
211  &  $-$18.81  &  $-$17.16  &  $-$18.54  &  40.74  &  5.3  &  $-$0.1  \\  %  52764-1321-044
212  &  $-$20.57  &  $-$18.55  &  $-$20.39  &  41.38  &  6.0  &  $-$0.2  \\  %  53091-1464-029
213  &  $-$21.06  &  $-$18.34  &  $-$20.96  &  41.29  &  5.8  &  $-$0.1  \\  %  51671-0299-134
214  &  $-$20.69  &  $-$18.55  &  $-$20.53  &  41.39  &  6.1  &  $-$0.4  \\  %  52762-1283-635
215  &  $-$20.11  &  $-$17.59  &  $-$20.00  &  40.94  &  6.2  &  $-$0.8  \\  %  51943-0300-281
216  &  $-$19.43  &  $-$16.15  &  $-$19.38  &  40.28  &  6.3  &  $-$1.5  \\  %  52079-0604-536
217  &  $-$20.71  &  $-$17.85  &  $-$20.63  &  41.06  &  5.6  &  $-$0.2  \\  %  52736-1284-151
218  &  $-$19.66  &  $-$16.41  &  $-$19.61  &  40.39  &  5.8  &  $-$1.0  \\  %  52026-0530-183
219  &  $-$20.18  &  $-$17.39  &  $-$20.09  &  40.85  &  6.2  &  $-$1.0  \\  %  52026-0530-541
220  &  $-$20.31  &  $-$18.13  &  $-$20.16  &  41.19  &  5.8  &  $-$0.2  \\  %  51984-0498-344
221  &  $-$20.15  &  $-$18.88  &  $-$19.74  &  41.54  &  6.2  &  $-$0.3  \\  %  51989-0497-014
222  &  $-$19.40  &  $-$16.36  &  $-$19.33  &  40.37  &  6.3  &  $-$1.4  \\  %  52443-0915-437
223  &  $-$18.56  &  $-$17.88  &  $-$17.73  &  41.07  &  6.3  &  $-$0.8  \\  %  51688-0302-227
224  &  $-$20.72  &  $-$17.85  &  $-$20.64  &  41.06  &  6.2  &  $-$0.7  \\  %  53178-1704-481
225  &  $-$21.03  &  $-$18.68  &  $-$20.90  &  41.44  &  5.9  &  $-$0.2  \\  %  51615-0303-302
226  &  $-$21.50  &  $-$17.86  &  $-$21.47  &  41.07  &  6.1  &  $-$0.6  \\  %  53108-1394-391
227  &  $-$21.64  &  $-$17.72  &  $-$21.61  &  41.00  &  6.0  &  $-$0.6  \\  %  51615-0303-435
228  &  $-$18.75  &  $-$15.84  &  $-$18.68  &  40.13  &  5.9  &  $-$1.2  \\  %  52055-0583-174
229  &  $-$20.82  &  $-$18.25  &  $-$20.71  &  41.25  &  5.9  &  $-$0.3  \\  %  52728-1287-365
230  &  $-$20.00  &  $-$18.52  &  $-$19.68  &  41.37  &  6.0  &  $-$0.3  \\  %  51988-0499-293
231  &  $-$20.68  &  $-$16.88  &  $-$20.65  &  40.61  &  6.0  &  $-$1.0  \\  %  52365-0606-565
232  &  $-$20.05  &  $-$18.55  &  $-$19.73  &  41.39  &  6.2  &  $-$0.5  \\  %  51997-0534-047
233  &  $-$20.51  &  $-$18.87  &  $-$20.24  &  41.53  &  6.3  &  $-$0.4  \\  %  53144-1644-094
234  &  $-$21.24  &  $-$16.25  &  $-$21.23  &  40.32  &  5.9  &  $-$1.1  \\  %  53144-1644-048
235  &  $-$20.49  &  $-$17.69  &  $-$20.40  &  40.98  &  6.2  &  $-$0.8  \\  %  52441-0790-230
236  &  $-$20.48  &  $-$16.94  &  $-$20.43  &  40.64  &  6.2  &  $-$1.2  \\  %  52441-0790-253
237  &  $-$20.46  &  $-$19.02  &  $-$20.13  &  41.60  &  6.2  &  $-$0.2  \\  %  52731-1288-430
238  &  $-$19.09  &  $-$16.28  &  $-$19.01  &  40.33  &  6.0  &  $-$1.2  \\  %  52781-1327-377
239  &  $-$20.02  &  $-$15.41  &  $-$20.01  &  39.93  &  5.7  &  $-$1.2  \\  %  52023-0586-234
240  &  $-$21.51  &  $-$17.81  &  $-$21.48  &  41.04  &  5.8  &  $-$0.3  \\  %  52409-0919-223
241  &  $-$21.00  &  $-$18.92  &  $-$20.83  &  41.56  &  5.9  &  $ $0.0  \\  %  52441-0790-156
242  &  $-$18.49  &  $-$15.77  &  $-$18.39  &  40.10  &  5.7  &  $-$1.1  \\  %  53172-1645-139
243  &  $-$20.47  &  $-$15.33  &  $-$20.46  &  39.90  &  6.2  &  $-$1.8  \\  %  52409-0919-512
244  &  $-$20.60  &  $-$18.49  &  $-$20.43  &  41.36  &  6.1  &  $-$0.4  \\  %  52668-1162-156
245  &  $-$20.44  &  $-$17.34  &  $-$20.38  &  40.82  &  6.1  &  $-$0.8  \\  %  52411-0920-289
246  &  $-$20.77  &  $-$17.23  &  $-$20.73  &  40.78  &  5.8  &  $-$0.5  \\  %  53172-1645-626
247  &  $-$18.60  &  $-$16.00  &  $-$18.50  &  40.20  &  6.1  &  $-$1.4  \\  %  52081-0608-405
248  &  $-$18.96  &  $-$17.45  &  $-$18.65  &  40.88  &  6.3  &  $-$1.0  \\  %  51662-0308-492
249  &  $-$20.60  &  $-$18.92  &  $-$20.34  &  41.56  &  6.3  &  $-$0.4  \\  %  52435-0791-511
250  &  $-$21.00  &  $-$18.39  &  $-$20.90  &  41.31  &  6.1  &  $-$0.4  \\  %  51994-0309-071
251  &  $-$20.72  &  $-$16.63  &  $-$20.69  &  40.50  &  6.1  &  $-$1.1  \\  %  53147-1676-530
252  &  $-$21.47  &  $-$18.46  &  $-$21.40  &  41.35  &  5.9  &  $-$0.2  \\  %  53108-1385-233
253  &  $-$20.64  &  $-$18.71  &  $-$20.44  &  41.46  &  6.2  &  $-$0.4  \\  %  52703-1165-424
254  &  $-$19.86  &  $-$17.42  &  $-$19.74  &  40.86  &  6.2  &  $-$1.0  \\  %  52426-0922-589
255  &  $-$21.50  &  $-$19.47  &  $-$21.32  &  41.81  &  6.0  &  $ $0.1  \\  %  52057-0590-103
256  &  $-$20.60  &  $-$18.30  &  $-$20.46  &  41.27  &  6.1  &  $-$0.4  \\  %  53116-1386-550
257  &  $-$21.68  &  $-$17.92  &  $-$21.65  &  41.09  &  5.8  &  $-$0.3  \\  %  52765-1293-387
258  &  $-$21.05  &  $-$16.92  &  $-$21.03  &  40.63  &  6.0  &  $-$0.9  \\  %  52736-1292-026
259  &  $-$21.71  &  $-$17.86  &  $-$21.67  &  41.07  &  5.6  &  $-$0.1  \\  %  52376-0794-550
260  &  $-$20.30  &  $-$17.85  &  $-$20.18  &  41.06  &  6.3  &  $-$0.8  \\  %  52411-0925-266
261  &  $-$17.76  &  $-$15.44  &  $-$17.62  &  39.94  &  4.9  &  $-$0.4  \\  %  52026-0593-547
262  &  $-$19.45  &  $-$16.73  &  $-$19.35  &  40.54  &  6.1  &  $-$1.1  \\  %  53119-1388-039
263  &  $-$21.38  &  $-$18.07  &  $-$21.33  &  41.16  &  6.2  &  $-$0.6  \\  %  53135-1389-611
264  &  $-$19.86  &  $-$18.26  &  $-$19.58  &  41.25  &  6.1  &  $-$0.5  \\  %  52045-0594-216
265  &  $-$20.23  &  $-$17.72  &  $-$20.11  &  41.00  &  6.2  &  $-$0.8  \\  %  52731-1168-417
266  &  $-$19.46  &  $-$18.86  &  $-$18.53  &  41.53  &  6.2  &  $-$0.3  \\  %  52782-1333-153
267  &  $-$20.75  &  $-$17.04  &  $-$20.72  &  40.69  &  5.4  &  $-$0.2  \\  %  52516-1054-128
268  &  $-$20.31  &  $-$16.27  &  $-$20.28  &  40.33  &  6.0  &  $-$1.2  \\  %  52761-1055-086
269  &  $-$20.20  &  $-$18.65  &  $-$19.90  &  41.43  &  6.3  &  $-$0.5  \\  %  51690-0345-601
270  &  $-$20.24  &  $-$16.45  &  $-$20.20  &  40.41  &  5.8  &  $-$0.9  \\  %  51693-0346-147
271  &  $-$19.55  &  $-$17.58  &  $-$19.36  &  40.94  &  5.9  &  $-$0.6  \\  %  52764-1056-067
272  &  $-$19.99  &  $-$15.17  &  $-$19.97  &  39.82  &  6.3  &  $-$1.9  \\  %  52759-1172-346
273  &  $-$21.10  &  $-$18.83  &  $-$20.96  &  41.51  &  6.2  &  $-$0.4  \\  %  53146-1420-093
274  &  $-$20.73  &  $-$16.17  &  $-$20.71  &  40.28  &  5.9  &  $-$1.2  \\  %  52000-0364-259
275  &  $-$20.29  &  $-$18.33  &  $-$20.09  &  41.28  &  6.0  &  $-$0.4  \\  %  52000-0364-128
276  &  $-$20.24  &  $-$16.40  &  $-$20.21  &  40.39  &  5.4  &  $-$0.5  \\  %  52522-1057-630
277  &  $-$21.26  &  $-$19.32  &  $-$21.06  &  41.74  &  6.2  &  $-$0.2  \\  %  52057-0626-433
278  &  $-$19.00  &  $-$17.43  &  $-$18.71  &  40.86  &  5.8  &  $-$0.5  \\  %  53177-1572-457
279  &  $-$20.08  &  $-$19.00  &  $-$19.57  &  41.59  &  6.2  &  $-$0.3  \\  %  52144-0627-631
280  &  $-$20.95  &  $-$16.01  &  $-$20.94  &  40.21  &  5.4  &  $-$0.6  \\  %  52144-0627-604
281  &  $-$17.41  &  $-$17.10  &  $-$15.91  &  40.71  &  6.3  &  $-$1.1  \\  %  52912-1424-260
282  &  $-$21.27  &  $-$18.97  &  $-$21.13  &  41.58  &  6.3  &  $-$0.4  \\  %  51699-0349-364
283  &  $-$21.41  &  $-$18.90  &  $-$21.29  &  41.55  &  6.2  &  $-$0.3  \\  %  51703-0353-460
284  &  $-$18.85  &  $-$18.02  &  $-$18.18  &  41.14  &  6.0  &  $-$0.5  \\  %  51691-0350-263
285  &  $-$20.06  &  $-$17.53  &  $-$19.95  &  40.91  &  6.2  &  $-$0.8  \\  %  51997-0367-298
286  &  $-$19.93  &  $-$17.77  &  $-$19.77  &  41.02  &  6.0  &  $-$0.6  \\  %  51788-0355-585
287  &  $-$19.33  &  $-$17.91  &  $-$18.98  &  41.09  &  5.9  &  $-$0.4  \\  %  51821-0359-535
288  &  $-$20.78  &  $-$18.63  &  $-$20.62  &  41.42  &  5.9  &  $-$0.2  \\  %  52443-0983-382
289  &  $-$19.52  &  $-$18.58  &  $-$18.94  &  41.40  &  6.2  &  $-$0.4  \\  %  52176-0636-105
290  &  $-$19.52  &  $-$16.75  &  $-$19.43  &  40.55  &  6.1  &  $-$1.1  \\  %  52431-0985-396
291  &  $-$21.04  &  $-$17.32  &  $-$21.00  &  40.81  &  5.6  &  $-$0.4  \\  %  52520-0728-179
292  &  $-$19.65  &  $-$17.04  &  $-$19.55  &  40.69  &  6.3  &  $-$1.2  \\  %  52520-0728-563
293  &  $-$19.86  &  $-$17.44  &  $-$19.74  &  40.87  &  6.2  &  $-$0.9  \\  %  52178-0640-252
294  &  $-$18.97  &  $-$15.57  &  $-$18.92  &  40.01  &  6.0  &  $-$1.5  \\  %  52199-0641-531
295  &  $-$21.34  &  $-$16.93  &  $-$21.32  &  40.63  &  5.9  &  $-$0.8  \\  %  51791-0374-287
296  &  $-$20.54  &  $-$17.32  &  $-$20.48  &  40.81  &  5.9  &  $-$0.7  \\  %  52206-0718-608
297  &  $-$21.11  &  $-$19.22  &  $-$20.90  &  41.69  &  6.1  &  $-$0.1  \\  %  52520-0739-416
298  &  $-$20.21  &  $-$18.21  &  $-$20.02  &  41.23  &  6.3  &  $-$0.7  \\  %  52263-0742-353
299  &  $-$20.20  &  $-$16.88  &  $-$20.15  &  40.61  &  6.2  &  $-$1.2  \\  %  51811-0381-363
300  &  $-$21.21  &  $-$17.07  &  $-$21.19  &  40.70  &  6.3  &  $-$1.2  \\  %  52262-0743-506
301  &  $-$20.04  &  $-$17.94  &  $-$19.87  &  41.10  &  6.3  &  $-$0.8  \\  %  52226-0726-257
302  &  $-$21.35  &  $-$19.91  &  $-$21.02  &  42.01  &  6.3  &  $-$0.0  \\  %  52523-0646-560
303  &  $-$19.26  &  $-$15.26  &  $-$19.23  &  39.86  &  5.5  &  $-$1.1  \\  %  51877-0385-264
304  &  $-$21.17  &  $-$19.25  &  $-$20.97  &  41.71  &  6.3  &  $-$0.3  \\  %  51877-0385-379
305  &  $-$20.67  &  $-$17.27  &  $-$20.62  &  40.79  &  6.1  &  $-$0.8  \\  %  51877-0385-121
306  &  $-$19.52  &  $-$16.79  &  $-$19.43  &  40.57  &  6.1  &  $-$1.1  \\  %  52559-0648-572
307  &  $-$20.82  &  $-$17.82  &  $-$20.75  &  41.04  &  6.1  &  $-$0.7  \\  %  52226-0749-439
308  &  $-$20.49  &  $-$16.85  &  $-$20.45  &  40.60  &  6.3  &  $-$1.2  \\  %  51788-0386-197
309  &  $-$20.40  &  $-$16.46  &  $-$20.37  &  40.42  &  6.0  &  $-$1.1      %  51791-0387-432

